Tonal coarticulation revisited: functional covariance analysis to investigate the planning of co-articulated tones by Standard Chinese speakers

We aim to explain whether a stress memory task has a significant impact on tonal coarticulation. We contribute a novel approach to analyse tonal coarticulation in phonetics, where several f0 contours are compared with respect to their vibrations at higher resolution, something that in statistical terms is called variation of the second order. We identify speech recording frequency curves as functional observations and harness inspiration from the mathematical fields of functional data analysis and optimal transport. By leveraging results from these two disciplines, we make one key observation:we identify the time and frequency covariance functions as crucial features for capturing the finer effects of tonal coarticulation. This observation leads us to propose a 2 steps approach where the mean functions are modelled via Generalized Additive Models, and the residuals of such models are investigated for any structure nested at covariance level. If such structure exist, we describe the variation manifested by the covariances through covariance principal component analysis. The 2-steps approach allows to uncover any variation not explained by generalized additive modelling, as well as fill a known shortcoming of these models into incorporating complex correlation structures in the data. The proposed method is illustrated on an articulatory dataset contrasting the pronunciation non-sensical bi-syllabic combinations in the presence of a short-memory challenge

==> biblio.tex <==




%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for David Kraus at 2012-05-14 10:56:13 +0200 


%% Saved with string encoding Unicode (UTF-8) 


@string{academic = {Academic Press, New York}}

@string{annap = {Ann. Appl. Probab.}}

@string{annms = {Ann. Math. Statist.}}

@string{annst = {Ann. Statist.}}

@string{biomk = {Biometrika}}

@string{bioms = {Biometrics}}

@string{birk = {{Birkh\"auser, Boston}}}

@string{cambridge = {{Cambridge University Press, Cambridge}}}

@string{chapmanhall = {{Chapman \& Hall, London--NewYork}}}

@string{csda = {Comput. Statist. Data Anal.}}

@string{isr = {Int. Stat. Rev.}}

@string{jasa = {J.~Amer. Statist. Assoc.}}

@string{jmva = {J.~Multivariate Anal.}}

@string{jrssb = {J. Roy. Statist. Soc. Ser.~B}}

@string{kluwerboston = {{Kluwer, Boston}}}

@string{kluwerdordrecht = {{Kluwer Acad. Press, Dordrecht}}}

@string{kyb = {Kybernetika}}

@string{lida = {Lifetime Data Anal.}}

@string{oxfordny = {{Oxford University Press, New York}}}

@string{scajs = {Scand. J.~Statist.}}

@string{sisp = {Statistical Inference for Stochastic Processes}}

@string{spl = {Statist. Probab. Lett.}}

@string{springer = {Springer, New York}}

@string{statdec = {Statist. Decisions}}

@string{statmed = {Stat. Med.}}

@string{stpra = {Stochastic Process. Appl.}}

@string{techn = {Technometrics}}

@string{teovp = {Teor. Veroyatnost. i Primenen.}}

@string{thepa = {Theory Probab. Appl.}}

@string{wiley = {Wiley, New York}}

@article{tavakoli2024statistics,
  title={Statistics in Phonetics},
  author={Tavakoli, Shahin and Matteo, Beatrice and Pigoli, Davide and Chodroff, Eleanor and Coleman, John and Gubian, Michele and Renwick, Margaret EL and Sonderegger, Morgan},
  journal={arXiv preprint arXiv:2404.07567},
  year={2024}
}

@article{silverman1996smoothed,
  title={Smoothed functional principal components analysis by choice of norm},
  author={Silverman, Bernard W},
  journal={The Annals of Statistics},
  volume={24},
  number={1},
  pages={1--24},
  year={1996},
  publisher={Institute of Mathematical Statistics}
}

@article{ocana1999functional,
  title={Functional principal components analysis by choice of norm},
  author={Oca{\~n}a, Francisco Antonio and Aguilera, Ana M and Valderrama, Mariano J},
  journal={Journal of Multivariate Analysis},
  volume={71},
  number={2},
  pages={262--276},
  year={1999},
  publisher={Elsevier}
}


@article{jones1941berkeley,
  title={The Berkeley growth study},
  author={Jones, Harold E and Bayley, Nancy},
  journal={Child development},
  pages={167--173},
  year={1941},
  publisher={JSTOR}
}


@article{douglas1966majorization,
  title={On majorization, factorization, and range inclusion of operators on Hilbert space},
  author={Douglas, Ronald G},
  journal={Proceedings of the American Mathematical Society},
  volume={17},
  number={2},
  pages={413--415},
  year={1966},
  publisher={JSTOR}
}

@book{zhang2013analysis,
  title={Analysis of variance for functional data},
  author={Zhang, Jin-Ting},
  year={2013},
  publisher={Chapman and Hall/CRC}
}

@article{bhatia,
title = "On the {B}ures-{W}asserstein distance between positive definite matrices",
journal = "Expositiones Mathematicae (in press, https://doi.org/10.1016/j.exmath.2018.01.002)",
year = "2018",
issn = "0723-0869",
doi = "https://doi.org/10.1016/j.exmath.2018.01.002",
url = "http://www.sciencedirect.com/science/article/pii/S0723086918300021",
author = "Rajendra Bhatia and Tanvi Jain and Yongdo Lim",
keywords = "Positive definite matrices, Bures distance, Wasserstein metric, Optimal transport, Coupling problem, Fidelity"
}


@article{masarotto2018procrustes,
  title={Procrustes Metrics on Covariance Operators and Optimal Transportation of Gaussian Processes},
  author={Masarotto, Valentina and Panaretos, Victor M and Zemel, Yoav},
  journal={Sankhya A},
  pages={1--42},
  year={2018},
  publisher={Springer}
}


@article{panaretos2016amplitude,
  title={Amplitude and phase variation of point processes},
  author={Panaretos, Victor M and Zemel, Yoav},
  journal={The Annals of Statistics},
  volume={44},
  number={2},
  pages={771--812},
  year={2016},
  publisher={Institute of Mathematical Statistics}
}


@book{panaretos2020invitation,
  title={An invitation to statistics in Wasserstein space},
  author={Panaretos, Victor M and Zemel, Yoav},
  year={2020},
  publisher={Springer Nature}
}


@phdthesis{zemel2017thesis,
  title={Fr{\'e}chet means in {W}asserstein space:  theory and algorithms},
    school   = {\'Ecole Polytechnique F\'ed\'erale de Lausanne},
  author={Zemel, Yoav},
    year     = {2017}
}


@article{ruschendorf1990characterization,
  title={A characterization of random variables with minimum {$L^2$}-distance},
  author={R{\"u}schendorf, L{\"u}dger and Rachev, Svetlozar T},
  journal={Journal of Multivariate Analysis},
  volume={32},
  number={1},
  pages={48--54},
  year={1990},
  publisher={Elsevier}
}

@article{cuesta1989notes,
  title={Notes on the {W}asserstein metric in {H}ilbert spaces},
  author={Cuesta-Albertos, Juan Antonio and Matr{\'a}n, Carlos},
  journal={The Annals of Probability},
  volume={17},
  number={3},
  pages={1264--1276},
  year={1989},
  publisher={JSTOR}
}

@book{van1996weak,
  title={Weak Convergence and Empirical Processes},
  author={van der Vaart, Aad W and Wellner, Jon A},
  year={1996},
  publisher={Springer}
}

@book{villani2003topics,
	Author = {C\'{e}dric Villani},
	Publisher = {American Mathematical Society},
	Title = {Topics in Optimal Transportation},
	Volume = {58},
	Year = {2003}
	}

@article{brenier1987decomposition,
  title={D{\'e}composition polaire et r{\'e}arrangement monotone des champs de vecteurs},
  author={Brenier, Yann},
  journal={CR Acad. Sci. Paris S{\'e}r. I Math},
  volume={305},
  number={19},
  pages={805--808},
  year={1987}
}

@article{brenier1991polar,
  title={Polar factorization and monotone rearrangement of vector-valued functions},
  author={Brenier, Yann},
  journal={Communications on pure and applied mathematics},
  volume={44},
  number={4},
  pages={375--417},
  year={1991},
  publisher={Wiley Online Library}
}


@article{pigoli2014distances,
  title={Distances and inference for covariance operators},
  author={Pigoli, Davide and Aston, John AD and Dryden, Ian L and Secchi, Piercesare},
  journal={Biometrika},
  volume={101},
  number={2},
  pages={409--422},
  year={2014},
  publisher={Oxford University Press}
}

@article{agueh2011barycenters,
	Author = {Martial Agueh and Guillaume Carlier},
	Journal = {Society for Industrial and Applied Mathematics},
	Title = {Barycenters in the {W}asserstein space},
	Volume = {43},
	number = {2},
	Pages = {904--924},
	Year = {2011}
	}

@inproceedings{ziezold1977expected,
  title={On expected figures and a strong law of large numbers for random elements in quasi-metric spaces},
  author={Ziezold, Herbert},
  booktitle={Transactions of the Seventh Prague Conference on Information Theory, Statistical Decision Functions, Random Processes and of the 1974 European Meeting of Statisticians},
  pages={591--602},
  year={1977},
  organization={Springer}}

@book{baker1970covariance,
  title={On covariance operators},
  author={Baker, Charles R},
  year={1970},
  publisher={University of North Carolina, Department of Statistics}
}

@article{alvarez2016fixed,
  title={A fixed-point approach to barycenters in {W}asserstein space},
  author={{\'A}lvarez-Esteban, Pedro C and del Barrio, E and Cuesta-Albertos, JA and Matr{\'a}n, C},
  journal={Journal of Mathematical Analysis and Applications},
  volume={441},
  number={2},
  pages={744--762},
  year={2016},
  publisher={Elsevier}
}

@article{dowson1982frechet,
  title={The {F}r{\'e}chet distance between multivariate normal distributions},
  author={Dowson, DC and Landau, BV},
  journal={Journal of multivariate analysis},
  volume={12},
  number={3},
  pages={450--455},
  year={1982},
  publisher={Elsevier}
}

@book{bogachev1998gaussian,
  title={Gaussian measures},
  author={Bogachev, Vladimir Igorevich},
  volume={62},
  year={1998},
  publisher={American Mathematical Society Providence}
}

@article{gouic2016existence,
  title={Existence and consistency of {W}asserstein barycenters},
  author={Le Gouic, Thibaut and Loubes, Jean-Michel},
  journal={Probability Theory and Related Fields},
  pages={1--17},
  year={2016},
  publisher={Springer}
}

@book{stein2009real,
  title={Real analysis: measure theory, integration, and {H}ilbert spaces},
  author={Stein, Elias M and Shakarchi, Rami},
  year={2009},
  publisher={Princeton University Press}
}

@article{cuesta1996lower,
  title={On lower bounds for the $L_2$-{W}asserstein metric in a {H}ilbert space},
  author={Cuesta-Albertos, JA and Matr{\'a}n-Bea, C and Tuero-Diaz, A},
  journal={Journal of Theoretical Probability},
  volume={9},
  number={2},
  pages={263--283},
  year={1996},
  publisher={Springer}}

@book{huber-ronchetti-2009,
	Address = {Hoboken},
	Author = {Huber, Peter J. and Ronchetti, Elvezio M.},
	Date-Added = {2012-05-11 13:14:23 +0200},
	Date-Modified = {2012-05-14 10:54:50 +0200},
	Doi = {10.1002/9780470434697},
	Publisher = {Wiley},
	Title = {Robust Statistics},
	Url = {http://dx.doi.org/10.1002/9780470434697},
	Year = {2009},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2488795}}

@article{bali-etal-2012,
	Author = {Bali, L. and Boente, G. and Tyler, D. E. and Wang, J.-L.},
	Date-Added = {2012-01-30 15:42:46 +0100},
	Date-Modified = {2012-01-30 15:43:57 +0100},
	Journal = {Ann. Statist.},
	Pages = {2852--2882},
	Title = {Robust Functional Principal Components: a projection-pursuit approach},
	Volume = {39},
	Year = {2012}}

@book{huber-1981,
	Address = {New York},
	Author = {Huber, Peter J.},
	Date-Added = {2011-12-06 21:50:26 +0100},
	Date-Modified = {2012-05-14 10:54:39 +0200},
	Publisher = {Wiley},
	Title = {Robust Statistics},
	Year = {1981},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=606374}}

@article{fritz-etal-2011,
	Author = {Heinrich Fritz and Peter Filzmoser and Christophe Croux},
	Date-Added = {2011-12-06 21:41:01 +0100},
	Date-Modified = {2012-05-01 21:47:42 +0200},
	Doi = {10.1007/s00180-011-0262-4},
	Journal = {Comput. Statist.},
	Pages = {to appear},
	Title = {A comparison of algorithms for the multivariate {$L_1$}-median},
	Year = {2011},
	Bdsk-Url-1 = {http://www.springerlink.com/content/c15x22j71t7370h2/fulltext.pdf},
	Bdsk-Url-2 = {http://dx.doi.org/10.1007/s00180-011-0262-4}}

@article{sirkia-2007,
	Author = {Sirki{{\"a}}, Seija and Taskinen, Sara and Oja, Hannu},
	Date-Added = {2011-12-06 21:30:29 +0100},
	Date-Modified = {2011-12-06 21:31:29 +0100},
	Doi = {10.1016/j.jmva.2007.06.005},
	Fjournal = {Journal of Multivariate Analysis},
	Journal = {J. Multivariate Anal.},
	Pages = {1611--1629},
	Title = {Symmetrised {M}-estimators of multivariate scatter},
	Url = {http://dx.doi.org/10.1016/j.jmva.2007.06.005},
	Volume = {98},
	Year = {2007},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2370110}}

@article{sirkia-etal-2009,
	Author = {Sirki{{\"a}}, Seija and Taskinen, Sara and Oja, Hannu and Tyler, David E.},
	Date-Added = {2011-12-06 21:27:39 +0100},
	Date-Modified = {2011-12-06 21:28:30 +0100},
	Doi = {10.1080/10485250802495691},
	Fjournal = {Journal of Nonparametric Statistics},
	Journal = {J. Nonparametr. Stat.},
	Pages = {155--176},
	Title = {Tests and estimates of shape based on spatial signs and ranks},
	Url = {http://dx.doi.org/10.1080/10485250802495691},
	Volume = {21},
	Year = {2009},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2488152}}

@article{serfling-2004,
	Author = {Serfling, Robert},
	Date-Added = {2011-12-06 21:24:31 +0100},
	Date-Modified = {2011-12-06 21:26:18 +0100},
	Doi = {10.1016/S0378-3758(03)00156-3},
	Fjournal = {Journal of Statistical Planning and Inference},
	Journal = {J. Statist. Plann. Inference},
	Pages = {259--278},
	Title = {Nonparametric multivariate descriptive measures based on spatial quantiles},
	Url = {http://dx.doi.org/10.1016/S0378-3758(03)00156-3},
	Volume = {123},
	Year = {2004},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2062982}}

@article{ibazizen-2003,
	Author = {Ibazizen, Mohamed and Dauxois, Jacques},
	Date-Added = {2011-10-10 11:51:10 +0200},
	Date-Modified = {2011-10-10 11:51:47 +0200},
	Doi = {10.1080/0233188031000065442},
	Journal = {Statistics},
	Pages = {73--83},
	Title = {A robust principal component analysis},
	Url = {http://dx.doi.org/10.1080/0233188031000065442},
	Volume = {37},
	Year = {2003},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=1959897}}

@incollection{panaretos-etal-2011,
	Address = {Heidelberg},
	Author = {Victor M. Panaretos and David Kraus and John H. Maddocks},
	Booktitle = {Recent Advances in Functional Data Analysis and Related Topics},
	Date-Added = {2011-10-10 11:37:36 +0200},
	Date-Modified = {2012-05-14 10:56:13 +0200},
	Editor = {Fr{\'e}d{\'e}ric Ferraty},
	Pages = {245--250},
	Publisher = {Physica-Verlag},
	Title = {Second-Order Inference for Functional Data with Application to {DNA} Minicircles},
	Year = {2011}}

@incollection{boente-etal-2011,
	Address = {Heidelberg},
	Author = {Graciela Boente and Daniela Rodriguez and Mariela Sued},
	Booktitle = {Recent Advances in Functional Data Analysis and Related Topics},
	Date-Added = {2011-10-10 11:06:08 +0200},
	Date-Modified = {2012-05-14 10:56:01 +0200},
	Editor = {Fr{\'e}d{\'e}ric Ferraty},
	Pages = {49--53},
	Publisher = {Physica-Verlag},
	Title = {Testing the equality of covariance operators},
	Year = {2011}}

@article{panaretos-etal-2010,
	Author = {Panaretos, Victor M. and Kraus, David and Maddocks, John H.},
	Date-Added = {2011-10-07 13:55:23 +0200},
	Date-Modified = {2011-10-07 13:56:17 +0200},
	Doi = {10.1198/jasa.2010.tm09239},
	Journal = {J. Amer. Statist. Assoc.},
	Pages = {670--682},
	Title = {Second-order comparison of {G}aussian random functions and the geometry of {DNA} minicircles},
	Url = {http://dx.doi.org/10.1198/jasa.2010.tm09239},
	Volume = {105},
	Year = {2010},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2724851}}

@article{bali-etal-2011,
	Author = {Bali, L. and Boente, G. and Tyler, D. E. and Wang, J.-L.},
	Date-Added = {2011-10-07 13:53:15 +0200},
	Date-Modified = {2011-10-07 14:00:35 +0200},
	Journal = {Ann. Statist.},
	Pages = {to appear},
	Title = {Robust Functional Principal Components: a projection-pursuit approach},
	Year = {2011}}

@article{hall-hosseini-nassab-2006,
	Author = {Hall, Peter and Hosseini-Nasab, Mohammad},
	Date-Added = {2011-10-07 11:15:15 +0200},
	Date-Modified = {2011-10-07 11:19:22 +0200},
	Doi = {10.1111/j.1467-9868.2005.00535.x},
	Fjournal = {Journal of the Royal Statistical Society. Series B. Statistical Methodology},
	Issn = {1369-7412},
	Journal = {J. Roy. Statist. Soc. Ser. B},
	Mrclass = {62H25 (62-07)},
	Mrnumber = {2212577},
	Pages = {109--126},
	Title = {On properties of functional principal components analysis},
	Url = {http://dx.doi.org/10.1111/j.1467-9868.2005.00535.x},
	Volume = {68},
	Year = {2006},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2212577}}

@book{kuttler-2011,
	Author = {Kuttler, K.},
	Date-Added = {2011-10-04 15:31:37 +0200},
	Date-Modified = {2011-10-04 15:41:56 +0200},
	Publisher = {\verb|http://www.math.byu.edu/~klkuttle/SobolevSpacesB.pdf|},
	Title = {Topics in analysis},
	Year = {2011}}

@book{dudley-1999,
	Address = {Cambridge},
	Author = {Dudley, R. M.},
	Date-Added = {2011-10-04 15:24:10 +0200},
	Date-Modified = {2011-10-04 15:25:59 +0200},
	Publisher = {Cambridge University Press},
	Title = {Uniform central limit theorems},
	Year = {1999},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=1720712}}

@article{kraus-panaretos-2011,
	Author = {Kraus, D. and Panaretos, V. M.},
	Date-Added = {2011-06-09 11:57:03 +0200},
	Date-Modified = {2011-06-09 11:59:26 +0200},
	Journal = {Submitted},
	Title = {Statistical inference on the second-order structure of functional data in the presence of influential observations},
	Year = {2011}}

@article{zhang-etal-1991,
	Author = {Zhang, Ji and Pantula, Sastry G. and Boos, Dennis D.},
	Date-Added = {2011-04-07 14:14:37 +0200},
	Date-Modified = {2011-04-07 14:15:18 +0200},
	Journal = {Biometrika},
	Pages = {787--795},
	Title = {Robust methods for testing the pattern of a single covariance matrix},
	Volume = {78},
	Year = {1991},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=1147015}}

@article{yao-lee-2006,
	Author = {Yao, Fang and Lee, Thomas C. M.},
	Date-Added = {2011-04-07 14:12:35 +0200},
	Date-Modified = {2011-04-07 14:13:27 +0200},
	Journal = {J. Roy. Statist. Soc. Ser. B},
	Pages = {3--25},
	Title = {Penalized spline models for functional principal component analysis},
	Volume = {68},
	Year = {2006},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2212572}}

@article{tiku-balakrishnan-1985,
	Author = {Tiku, M. L. and Balakrishnan, N.},
	Date-Added = {2011-04-07 14:09:00 +0200},
	Date-Modified = {2011-04-07 14:10:49 +0200},
	Journal = {Comm. Statist. Theory Methods},
	Pages = {3033--3051},
	Title = {Testing the equality of variance-covariance matrices the robust way},
	Volume = {14},
	Year = {1985},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=821103}}

@article{sun-genton-2011,
	Author = {Sun, Y. and Genton, M. G.},
	Date-Added = {2011-04-07 14:03:31 +0200},
	Date-Modified = {2011-10-10 15:05:16 +0200},
	Journal = {J. Comput. Graph. Statist.},
	Pages = {316--334},
	Title = {Functional Boxplots},
	Volume = {20},
	Year = {2011}}

@article{olson-1974,
	Abstract = {Monte Carlo methods were used to study the performance of the largest-root test, two trace-type tests and three determinantal tests in the fixed-effects MANOVA model when certain assumptions are violated. Results indicated that for protection against nonnormality and heterogeneity of covariance matrices, the largest-root test should be avoided, while the Pillai-Bartlett trace test may be recommended as the most robust of the MANOVA tests, with adequate power to detect true differences in a variety of situations.},
	Author = {Olson, Chester L.},
	Date-Added = {2011-04-07 12:18:29 +0200},
	Date-Modified = {2011-04-07 12:19:08 +0200},
	Journal = {J. Amer. Statist. Assoc.},
	Pages = {894--908},
	Title = {Comparative Robustness of Six Tests in Multivariate Analysis of Variance},
	Volume = {69},
	Year = {1974},
	Bdsk-Url-1 = {http://www.jstor.org/stable/2286159}}

@book{nelson-1969,
	Address = {Princeton},
	Author = {Nelson, Edward},
	Date-Added = {2011-04-07 12:06:17 +0200},
	Date-Modified = {2012-05-14 10:55:15 +0200},
	Publisher = {Princeton University Press},
	Title = {Topics in Dynamics. {I}: {F}lows},
	Year = {1969},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=0282379}}

@article{li-chen-1985,
	Author = {Li, G. and Chen, Z.},
	Date-Added = {2011-04-07 12:00:50 +0200},
	Date-Modified = {2011-04-07 12:04:20 +0200},
	Journal = {J. Amer. Statist. Assoc.},
	Title = {Projection-Pursuit Approach to Robust Dispersion Matrices and Principal Components: Primary Theory and {M}onte {C}arlo},
	Volume = {80},
	Year = {1985}}

@article{layard-1974,
	Author = {Layard, M. W. J.},
	Date-Added = {2011-04-07 11:54:28 +0200},
	Date-Modified = {2011-04-07 11:56:18 +0200},
	Journal = {Biometrika},
	Pages = {461--465},
	Title = {A {M}onte {C}arlo comparison of tests for equality of convariance matrices},
	Volume = {61},
	Year = {1974}}

@book{hampel-etal-1986,
	Address = {New York},
	Author = {Hampel, Frank R. and Ronchetti, Elvezio M. and Rousseeuw, Peter J. and Stahel, Werner A.},
	Date-Added = {2011-04-07 11:39:27 +0200},
	Date-Modified = {2012-05-14 10:54:23 +0200},
	Publisher = {Wiley},
	Title = {Robust Statistics},
	Year = {1986},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=829458}}

@article{hall-etal-2006,
	Author = {Hall, Peter and M{{\"u}}ller, Hans-Georg and Wang, Jane-Ling},
	Date-Added = {2011-04-07 11:36:27 +0200},
	Date-Modified = {2011-04-07 11:37:18 +0200},
	Journal = {Ann. Statist.},
	Pages = {1493--1517},
	Title = {Properties of principal component methods for functional and longitudinal data analysis},
	Volume = {34},
	Year = {2006},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2278365}}

@article{gervini-2006,
	Author = {Gervini, Daniel},
	Date-Added = {2011-04-07 11:34:30 +0200},
	Date-Modified = {2011-04-07 11:35:19 +0200},
	Journal = {J. Roy. Statist. Soc. Ser. B},
	Pages = {671--687},
	Title = {Free-knot spline smoothing for functional data},
	Volume = {68},
	Year = {2006},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2301014}}

@article{gabrys-kokoszka-2007,
	Author = {Gabrys, Robertas and Kokoszka, Piotr},
	Date-Added = {2011-04-07 11:32:32 +0200},
	Date-Modified = {2011-04-07 11:33:37 +0200},
	Journal = {J. Amer. Statist. Assoc.},
	Pages = {1338--1348},
	Title = {Portmanteau test of independence for functional observations},
	Volume = {102},
	Year = {2007},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2412554}}

@article{dauxois-etal-1982,
	Author = {Dauxois, J. and Pousse, A. and Romain, Y.},
	Date-Added = {2011-04-07 11:29:52 +0200},
	Date-Modified = {2011-04-07 11:30:48 +0200},
	Journal = {J. Multivariate Anal.},
	Pages = {136--154},
	Title = {Asymptotic theory for the principal component analysis of a vector random function: some applications to statistical inference},
	Volume = {12},
	Year = {1982},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=650934}}

@article{box-1953,
	Author = {Box, G. E. P.},
	Date-Added = {2011-04-07 11:27:24 +0200},
	Date-Modified = {2011-04-07 11:28:03 +0200},
	Journal = {Biometrika},
	Pages = {318--335},
	Title = {Non-normality and tests on variances},
	Volume = {40},
	Year = {1953},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=0058937}}

@article{boente-fraiman-1999,
	Author = {Boente, G. and Fraiman, R.},
	Date-Added = {2011-04-07 11:23:20 +0200},
	Date-Modified = {2011-10-07 12:19:28 +0200},
	Journal = {Test},
	Pages = {28--35},
	Title = {Comment on a~paper by {Locantore} et al.},
	Volume = {8},
	Year = {1999}}

@article{anderson-2006,
	Author = {Anderson, Marti J.},
	Date-Added = {2011-04-07 11:10:22 +0200},
	Date-Modified = {2011-04-07 11:12:53 +0200},
	Journal = {Biometrics},
	Pages = {245--253},
	Title = {Distance-based tests for homogeneity of multivariate dispersions},
	Volume = {62},
	Year = {2006},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2226579}}

@book{adler-1990,
	Address = {Hayward},
	Author = {Adler, Robert J.},
	Date-Added = {2011-04-07 11:07:45 +0200},
	Date-Modified = {2012-05-14 10:54:05 +0200},
	Publisher = {Institute of Mathematical Statistics},
	Series = {Institute of Mathematical Statistics Lecture Notes---Monograph Series, 12},
	Title = {An Introduction to Continuity, Extrema, and Related Topics for General {G}aussian Processes},
	Year = {1990},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=1088478}}

@article{amzallag-etal-2006,
	Author = {Arnaud Amzallag and C{\'e}dric Vaillant and Mathews Jacob and Michael Unser and Jan Bednar and Jason D. Kahn and Jacques Dubochet and Andrzej Stasiak and John H. Maddocks},
	Date-Added = {2011-04-05 14:40:27 +0200},
	Date-Modified = {2011-04-05 14:45:54 +0200},
	Journal = {Nucl. Acids Res.},
	Pages = {e125},
	Title = {{3D} reconstruction and comparison of shapes of {DNA} minicircles observed by cryo-electron microscopy},
	Volume = {34},
	Year = {2006}}

@article{chaudhuri-1996,
	Author = {Chaudhuri, Probal},
	Date-Added = {2011-04-03 22:33:17 +0200},
	Date-Modified = {2011-04-03 22:34:09 +0200},
	Journal = {J. Amer. Statist. Assoc.},
	Pages = {862--872},
	Title = {On a geometric notion of quantiles for multivariate data},
	Volume = {91},
	Year = {1996},
	Bdsk-Url-1 = {http://ams.org/mathscinet-getitem?mr=1395753}}

@article{marden-1999,
	Author = {Marden, John I.},
	Date-Added = {2011-01-28 09:56:01 +0100},
	Date-Modified = {2011-01-28 09:56:52 +0100},
	Journal = {Statist. Probab. Lett.},
	Pages = {349--359},
	Title = {Some robust estimates of principal components},
	Url = {http://dx.doi.org/10.1016/S0167-7152(98)00272-7},
	Volume = {43},
	Year = {1999},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=1707944}}

@article{yao-etal-2005b,
	Author = {Yao, Fang and M{\"u}ller, Hans-Georg and Wang, Jane-Ling},
	Date-Added = {2010-11-26 11:42:48 +0100},
	Date-Modified = {2010-11-26 11:45:19 +0100},
	Journal = {Ann. Statist.},
	Pages = {2873--2903},
	Title = {Functional linear regression analysis for longitudinal data},
	Url = {http://dx.doi.org/10.1214/009053605000000660},
	Volume = {33},
	Year = {2005},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2253106}}

@article{yao-etal-2005a,
	Author = {Yao, Fang and M{\"u}ller, Hans-Georg and Wang, Jane-Ling},
	Date-Added = {2010-11-26 11:42:08 +0100},
	Date-Modified = {2010-11-26 11:44:21 +0100},
	Journal = {J. Amer. Statist. Assoc.},
	Pages = {577--590},
	Title = {Functional data analysis for sparse longitudinal data},
	Url = {http://dx.doi.org/10.1198/016214504000001745},
	Volume = {100},
	Year = {2005},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2160561}}

@article{horvath-etal-2010,
	Author = {Horv\'ath, Lajos and Hu{\v{s}}kov\'a, Marie and Kokoszka, Piotr},
	Date-Added = {2010-11-26 11:30:51 +0100},
	Date-Modified = {2011-10-07 11:58:57 +0200},
	Journal = {J. Multivariate Anal.},
	Pages = {352--367},
	Title = {Testing the stability of the functional autoregressive process},
	Url = {http://dx.doi.org/10.1016/j.jmva.2008.12.008},
	Volume = {101},
	Year = {2010},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2564345}}

@article{cardot-etal-1999,
	Author = {Cardot, Herv{\'e} and Ferraty, Fr{\'e}d{\'e}ric and Sarda, Pascal},
	Date-Added = {2010-11-26 11:23:59 +0100},
	Date-Modified = {2010-11-26 11:25:21 +0100},
	Journal = {Statist. Probab. Lett.},
	Pages = {11--22},
	Title = {Functional linear model},
	Url = {http://dx.doi.org/10.1016/S0167-7152(99)00036-X},
	Volume = {45},
	Year = {1999},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=1718346}}

@article{cardot-etal-2003,
	Author = {Cardot, Herv{\'e} and Ferraty, Fr{\'e}d{\'e}ric and Mas, Andr{\'e} and Sarda, Pascal},
	Date-Added = {2010-11-26 11:23:44 +0100},
	Date-Modified = {2010-11-26 11:26:13 +0100},
	Journal = {Scand. J. Statist.},
	Pages = {241--255},
	Title = {Testing hypotheses in the functional linear model},
	Url = {http://dx.doi.org/10.1111/1467-9469.00329},
	Volume = {30},
	Year = {2003},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=1965105}}

@article{horvath-etal-2009,
	Author = {Horv\'ath, Lajos and Kokoszka, Piotr and Reimherr, Matthew},
	Date-Added = {2010-11-25 16:32:04 +0100},
	Date-Modified = {2010-11-25 16:33:30 +0100},
	Journal = {Canad. J. Statist.},
	Pages = {571--591},
	Title = {Two sample inference in functional linear models},
	Url = {http://dx.doi.org/10.1002/cjs.10035},
	Volume = {37},
	Year = {2009},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2588950}}

@article{benko-etal-2009,
	Author = {Benko, Michal and H\"ardle, Wolfgang and Kneip, Alois},
	Date-Added = {2010-11-25 15:07:02 +0100},
	Date-Modified = {2010-11-25 15:08:03 +0100},
	Journal = {Ann. Statist.},
	Pages = {1--34},
	Title = {Common functional principal components},
	Url = {http://dx.doi.org/10.1214/07-AOS516},
	Volume = {37},
	Year = {2009},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2488343}}

@article{james-sood-2006,
	Author = {James, Gareth M. and Sood, Ashish},
	Date-Added = {2010-11-25 14:52:21 +0100},
	Date-Modified = {2010-11-25 14:52:55 +0100},
	Journal = {Comput. Statist. Data Anal.},
	Pages = {1774--1792},
	Title = {Performing hypothesis tests on the shape of functional data},
	Url = {http://dx.doi.org/10.1016/j.csda.2005.02.010},
	Volume = {50},
	Year = {2006},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2222041}}

@article{berkes-etal-2009,
	Author = {Berkes, I. and Gabrys, R. and Horv\'ath, L. and Kokoszka, P.},
	Date-Added = {2010-11-25 14:45:25 +0100},
	Date-Modified = {2011-10-07 11:17:59 +0200},
	Journal = {J. Roy. Statist. Soc. Ser. B},
	Pages = {927--946},
	Title = {Detecting changes in the mean of functional observations},
	Volume = {71},
	Year = {2009}}

@article{cuevas-etal-2004,
	Author = {Cuevas, Antonio and Febrero, Manuel and Fraiman, Ricardo},
	Date-Added = {2010-11-25 14:27:46 +0100},
	Date-Modified = {2010-11-25 14:30:58 +0100},
	Journal = {Comput. Statist. Data Anal.},
	Pages = {111--122},
	Title = {An anova test for functional data},
	Url = {http://dx.doi.org/10.1016/j.csda.2003.10.021},
	Volume = {47},
	Year = {2004},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2087932}}

@article{locantore-etal-1999,
	Author = {Locantore, N. and Marron, J. S. and Simpson, D. G. and Tripoli, N. and Zhang, J. T. and Cohen, K. L.},
	Date-Added = {2010-09-02 17:41:24 +0200},
	Date-Modified = {2010-09-02 17:48:48 +0200},
	Journal = {Test},
	Pages = {1--73},
	Title = {Robust principal component analysis for functional data},
	Volume = {8},
	Year = {1999},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=1707596}}

@book{bosq-2000,
	Address = {New York},
	Author = {Bosq, D.},
	Date-Modified = {2012-05-14 10:53:31 +0200},
	Publisher = {Springer},
	Title = {Linear Processes in Function Spaces: Theory and Applications},
	Year = 2000}

@article{bigot2012consistent,
  title={Consistent estimation of a population barycenter in the {W}asserstein space},
  author={Bigot, J{\'e}r{\'e}mie and Klein, Thierry and others},
  journal={ArXiv e-prints},
  year={2012}
}

@article{bigot2012characterization,
  title={Characterization of barycenters in the {W}asserstein space by averaging optimal transport maps},
  author={Bigot, J{\'e}r{\'e}mie and Klein, Thierry},
  journal={arXiv preprint arXiv:1212.2562},
  year={2012}
}

@article{gower1975generalized,
  title={Generalized {P}rocrustes analysis},
  author={Gower, John C},
  journal={Psychometrika},
  volume={40},
  number={1},
  pages={33--51},
  year={1975},
  publisher={Springer}
}


@article{gervini-2008,
	Author = {Gervini, D.},
	Journal = BIOMK,
	Pages = {587--600},
	Title = {Robust functional estimation using the median and spherical principal components},
	Volume = 95,
	Year = 2008}

@article{mas-2007,
	Author = {Mas, A.},
	Journal = SISP,
	Pages = {147--163},
	Title = {Testing for the mean of random curves: a penalization approach},
	Volume = 10,
	Year = 2007}

@article{olkin1982distance,
  title={The distance between two random vectors with given dispersion matrices},
  author={Olkin, Ingram and Pukelsheim, Friedrich},
  journal={Linear Algebra and its Applications},
  volume={48},
  pages={257--263},
  year={1982},
  publisher={Elsevier}
}

@book{ambrosio2008gradient,
  title={Gradient flows: in metric spaces and in the space of probability measures},
  author={Ambrosio, Luigi and Gigli, Nicola and Savar{\'e}, Giuseppe},
  year={2008},
  publisher={Springer Science \& Business Media}
}

@book{ramsay-silverman-2005,
	Address = {New York},
	Author = {Ramsay, J. and Silverman, B. W.},
	Date-Modified = {2012-05-14 10:55:39 +0200},
	Publisher = {Springer},
	Title = {Functional Data Analysis},
	Year = 2005}

@book{dryden1998statistical,
  title={Statistical analysis of shape},
  author={Dryden, IL and Mardia, KV},
  year={1998},
  publisher={Wiley}
}

@incollection{ambrosio2013user,
  title={A user’s guide to optimal transport},
  author={Ambrosio, Luigi and Gigli, Nicola},
  booktitle={Modelling and optimisation of flows on networks},
  pages={1--155},
  year={2013},
  publisher={Springer}
}

@article{knott1984optimal,
  title={On the optimal mapping of distributions},
  author={Knott, Martin and Smith, Cyril S},
  journal={Journal of Optimization Theory and Applications},
  volume={43},
  number={1},
  pages={39--49},
  year={1984},
  publisher={Springer}
}


@article{zemel2019frechet,
  title={Fr{\'e}chet means and Procrustes analysis in Wasserstein space},
  author={Zemel, Yoav and Panaretos, Victor M},
  journal={Bernoulli},
  volume={25},
  number={2},
  pages={932--976},
  year={2019},
  publisher={Bernoulli Society for Mathematical Statistics and Probability}
}

@article{fletcher2004principal,
  title={Principal geodesic analysis for the study of nonlinear statistics of shape},
  author={Fletcher, P Thomas and Lu, Conglin and Pizer, Stephen M and Joshi, Sarang},
  journal={IEEE transactions on medical imaging},
  volume={23},
  number={8},
  pages={995--1005},
  year={2004},
  publisher={IEEE}
}

@article{dryden2009non,
  title={Non-Euclidean statistics for covariance matrices, with applications to diffusion tensor imaging},
  author={Dryden, Ian L and Koloydenko, Alexey and Zhou, Diwei},
  journal={The Annals of Applied Statistics},
  pages={1102--1123},
  year={2009},
  publisher={JSTOR}
}


@article{jolliffe2002principal,
  title={Principal component analysis and factor analysis},
  author={Jolliffe, Ian T},
  journal={Principal component analysis},
  pages={150--166},
  year={2002},
  publisher={Springer}
}

@article{obrien-1992,
	Abstract = {Normal-theory tests for common variance are very sensitive to departures from normality in both univariate and multivariate applications. For mild departures from normality and moderate sample size, nominal α = .01 produced Type I error rates in excess of .20 in simulation studies. Since a modification of Levene's test has been shown to perform well for the univariate problem, two multivariate generalizations of this test are proposed. Both procedures are robust to departures from normality, and are simple computationally. Comparisons of the power of these two procedures and a procedure proposed previously by Tiku and Balakrishnan (1985, Communications in Statistics-Theory and Methods 14, 3033-3051) indicate that the three methods should be viewed as complementary.},
	Author = {O'Brien, Peter C.},
	Date-Added = {2011-04-07 12:13:32 +0200},
	Date-Modified = {2011-04-07 12:14:11 +0200},
	Journal = {Biometrics},
	Pages = {819-827},
	Title = {Robust Procedures for Testing Equality of Covariance Matrices},
	Volume = {48},
	Year = {1992},
	Bdsk-Url-1 = {http://www.jstor.org/stable/2532347}}

@article{frechet1948elements,
  title={Les {\'e}l{\'e}ments al{\'e}atoires de nature quelconque dans un espace distanci{\'e}},
  author={Fr{\'e}chet, Maurice},
  journal={Ann. Inst. H. Poincar{\'e}},
  volume={10},
  number={3},
  pages={215--310},
  year={1948}
}

@article{gangbo1998optimal,
  title={Optimal maps for the multidimensional {M}onge--{K}antorovich problem},
	Author = {Gangbo, Wilfrid and \'{S}wi\c{e}ch, Andrzej},
  journal={Communications on pure and applied mathematics},
  volume={51},
  number={1},
  pages={23--45},
  year={1998}
}

@article{alvarez2011uniqueness,
  title={Uniqueness and approximate computation of optimal incomplete transportation plans},
  author={{\'A}lvarez-Esteban, PC and Del Barrio, E and Cuesta-Albertos, JA and Matr{\'a}n, C and others},
  Journal={Annales de l'Institut Henri Poincar{\'e}, Probabilit{\'e}s et Statistiques},
  volume={47},
  number={2},
  pages={358--375},
  year={2011},
  Publisher={Institut Henri Poincar{\'e}}
}

@article{huckemann2010intrinsic,
  title={Intrinsic shape analysis: Geodesic PCA for {R}iemannian manifolds modulo isometric {L}ie group actions},
  author={Huckemann, Stephan and Hotz, Thomas and Munk, Axel},
  journal={Statistica Sinica},
  pages={1--58},
  year={2010},
  publisher={JSTOR}
}

@article{takatsu2011wasserstein,
  title={Wasserstein geometry of {G}aussian measures},
  author={Takatsu, Asuka},
  journal={Osaka Journal of Mathematics},
  volume={48},
  number={4},
  pages={1005--1026},
  year={2011},
  publisher={Osaka University and Osaka City University, Departments of Mathematics}
}

@article{mccann1997convexity,
  title={A convexity principle for interacting gases},
  author={McCann, Robert J},
  journal={Advances in mathematics},
  volume={128},
  number={1},
  pages={153--179},
  year={1997},
  publisher={Elsevier}
}

@article{ruschendorf2002n,
  title={On the n-coupling problem},
  author={R{\"u}schendorf, Ludger and Uckelmann, Ludger},
  journal={Journal of multivariate analysis},
  volume={81},
  number={2},
  pages={242--258},
  year={2002},
  publisher={Elsevier}
}

@book{durrett2010probability,
  title={Probability: theory and examples},
  author={Durrett, Rick},
  year={2010},
  publisher={Cambridge university press}
}



%%%%%%%% ADDITIONAL REFERENCES FOR THE INTRODUCTION




@article{larotonda2007nonpositive,
	Author = {Larotonda, Gabriel},
	Journal = {Differential Geometry and its Applications},
	Number = {6},
	Pages = {679--700},
	Publisher = {Elsevier},
	Title = {Nonpositive curvature: a geometrical approach to Hilbert--Schmidt operators},
	Volume = {25},
	Year = {2007}}

@article{lemmens2013unique,
	Author = {Lemmens, Bas and Roelands, Mark},
	Journal = {arXiv preprint arXiv:1305.6643},
	Title = {Unique geodesics for Thompson's metric},
	Year = {2013}}

@article{bhattacharya2003large,
	Author = {Bhattacharya, Rabi and Patrangenaru, Vic},
	Date-Modified = {2015-03-29 12:44:59 +0000},
	Journal = {Annals of statistics},
	Pages = {1--29},
	Publisher = {JSTOR},
	Title = {Large sample theory of intrinsic and extrinsic sample means on manifolds: i},
	Year = {2003}}

@article{bhattacharya2005large,
	Author = {Bhattacharya, Rabi and Patrangenaru, Vic},
	Date-Modified = {2015-03-29 12:44:50 +0000},
	Journal = {Annals of statistics},
	Pages = {1225--1259},
	Publisher = {JSTOR},
	Title = {Large sample theory of intrinsic and extrinsic sample means on manifolds: ii},
	Year = {2005}}



@phdthesis{schwartzman2006random,
	Author = {Schwartzman, Armin},
	School = {Stanford University},
	Title = {Random ellipsoids and false discovery rates: Statistics for diffusion tensor imaging data},
	Year = {2006}}

@book{horvath2012inference,
	Author = {Horv{\'a}th, Lajos and Kokoszka, Piotr},
	Publisher = {Springer Science \& Business Media},
	Title = {Inference for functional data with applications},
	Volume = {200},
	Year = {2012}}

@article{kraus2014components,
	Author = {Kraus, David},
	Journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
	Publisher = {Wiley Online Library},
	Title = {Components and completion of partially observed functional data},
	Year = {2014}}

@article{coffey2011common,
	Author = {Coffey, N and Harrison, AJ and Donoghue, OA and Hayes, K},
	Journal = {Human movement science},
	Number = {6},
	Pages = {1144--1166},
	Publisher = {Elsevier},
	Title = {Common functional principal components analysis: A new approach to analyzing human movement data},
	Volume = {30},
	Year = {2011}}

@article{pigoli2014permutation,
	Author = {Pigoli, Davide and Aston, John AD and Dryden, Ian L and Secchi, Piercesare},
	Journal = {Contributions in infinite-dimensional statistics and related topics},
	Pages = {215},
	Publisher = {Societ{\`a} Editrice Esculapio},
	Title = {Permutation tests for comparison of co-variance operators},
	Year = {2014}}

@article{jaruvskova2013testing,
	Author = {Jaru{\v{s}}kov{\'a}, Daniela},
	Journal = {Journal of Statistical Planning and Inference},
	Number = {9},
	Pages = {1500--1511},
	Publisher = {Elsevier},
	Title = {Testing for a change in covariance operator},
	Volume = {143},
	Year = {2013}}

@article{horvath2013test,
	Author = {Horv{\'a}th, Lajos and Hu{\v{s}}kov{\'a}, Marie and Rice, Gregory},
	Journal = {Journal of Multivariate Analysis},
	Pages = {100--119},
	Publisher = {Elsevier},
	Title = {Test of independence for functional data},
	Volume = {117},
	Year = {2013}}

@article{paparoditis2014bootstrap,
	Author = {Paparoditis, Efstathios and Sapatinas, Theofanis},
	Journal = {arXiv preprint arXiv:1409.4317},
	Title = {Bootstrap-based testing for functional data},
	Year = {2014}}

@article{gabrys2010tests,
	Author = {Gabrys, Robertas and Horv{\'a}th, Lajos and Kokoszka, Piotr},
	Journal = {Journal of the American Statistical Association},
	Number = {491},
	Pages = {1113--1125},
	Publisher = {Taylor \& Francis},
	Title = {Tests for error correlation in the functional linear model},
	Volume = {105},
	Year = {2010}}

@article{fremdt2013testing,
	Author = {Fremdt, Stefan and Steinebach, Josef G and Horv{\'a}th, Lajos and Kokoszka, Piotr},
	Journal = {Scandinavian Journal of Statistics},
	Number = {1},
	Pages = {138--152},
	Publisher = {Wiley Online Library},
	Title = {Testing the equality of covariance operators in functional samples},
	Volume = {40},
	Year = {2013}}

@book{zhang:2013,
	Author = {Zhang, J.T.},
	Date-Added = {2015-03-26 13:41:09 +0000},
	Date-Modified = {2015-03-26 13:41:58 +0000},
	Publisher = {Chapman \& Hall},
	Series = {Monographs on statistics and applied probability},
	Title = {Analysis of Variance for Functional Data},
	Year = {2013}}

@article{arnaud,
	Author = {Amzallag, A. and Vaillant, C. and Jacob, C. and Unser, M. and Bednar, M. and Kahn, J.D. and Dubichet, J. and Stasiak, A. and Maddocks, J.H.},
	Date-Added = {2015-03-25 16:17:46 +0000},
	Date-Modified = {2015-03-25 16:19:10 +0000},
	Journal = {Nucleic Acides Research},
	Number = {18},
	Pages = {e125},
	Title = {3D Reconstruction and Comparison of Shapes of DNA Minicircles Observed by Cryo-Electron Microscopy},
	Volume = {34},
	Year = {2006}}

@article{pigoli:2014,
	Author = {Pigoli, Davide and Aston, John D. and Dryden, Ian L. and Secchi, Piercesare},
	Date-Added = {2015-03-22 13:22:10 +0000},
	Date-Modified = {2015-03-22 13:23:05 +0000},
	Journal = {Biometrika},
	Number = {2},
	Pages = {409-422},
	Title = {Distances and inference for covariance functions},
	Volume = {101},
	Year = {2014}}


	
	@article{tavakoli:2014,
  title={Detecting and localizing differences in functional time series dynamics: a case study in molecular biophysics},
  author={Tavakoli, Shahin and Panaretos, Victor M},
  journal={Journal of the American Statistical Association},
  volume={111},
  number={515},
  pages={1020--1035},
  year={2016},
  publisher={Taylor \& Francis}
}

@article{Panaretos_SPA,
	Author = {Victor M. Panaretos and Shahin Tavakoli},
	Journal = {Stochastic Processes and their Applications},
	Number = {7},
	Pages = {2779 - 2807},
	Title = {Cram\'er-Karhunen-Lo\`eve representation and harmonic principal component analysis of functional time series},
	Volume = {123},
	Year = {2013}}

@article{panaretos_jasa,
	Author = {Victor M. Panaretos and David Kraus and John H. Maddocks},
	Date = {2010-01-01},
	Issn = {0162-1459},
	Journal = {J. Amer. Statist. Assoc.},
	Number = {490},
	Pages = {670--682},
	Title = {Second-order comparison of Gaussian random functions and the geometry of DNA minicircles},
	Url = {http://dx.doi.org/10.1198/jasa.2010.tm09239},
	Volume = {105},
	Year = {2010},
	Bdsk-Url-1 = {http://dx.doi.org/10.1198/jasa.2010.tm09239}}

@article{panaretos_biometrika,
	Author = {David Kraus and Victor M. Panaretos},
	Date = {2012-01-01},
	Journal = {Biometrika},
	Number = {4},
	Pages = {813--832},
	Title = {Dispersion operators and resistant second-order functional data analysis},
	Url = {http://dx.doi.org/10.1093/biomet/ass037},
	Volume = {99},
	Year = {2012},
	Bdsk-Url-1 = {http://dx.doi.org/10.1093/biomet/ass037}}

@article{hsu,
	Added-At = {2011-11-21T00:00:00.000+0100},
	Author = {Hsu, Daniel and Kakade, Sham M. and Zhang, Tong},
	Biburl = {http://www.bibsonomy.org/bibtex/2044b6309fd99d204da6cfac83f8a067d/dblp},
	Ee = {http://dx.doi.org/10.1109/TIT.2011.2158250},
	Interhash = {f4f3a0ecff514f53b060e378eff13d75},
	Intrahash = {044b6309fd99d204da6cfac83f8a067d},
	Journal = {IEEE Transactions on Information Theory},
	Keywords = {dblp},
	Number = 11,
	Pages = {7221-7234},
	Timestamp = {2011-11-21T00:00:00.000+0100},
	Title = {Robust Matrix Decomposition With Sparse Corruptions.},
	Url = {http://dblp.uni-trier.de/db/journals/tit/tit57.html#HsuKZ11},
	Volume = 57,
	Year = 2011,
	Bdsk-Url-1 = {http://dblp.uni-trier.de/db/journals/tit/tit57.html#HsuKZ11}}

@article{Agarwal,
	Author = {Agarwal, Alekh and Negahban, Sahand and Wainwright, Martin J},
	Journal = {The Annals of Statistics},
	Number = {2},
	Pages = {1171-1197},
	Publisher = {Institute of Mathematical Statistics, Beachwood, OH},
	Title = {Noisy matrix decomposition via convex relaxation: Optimal rates in high dimensions},
	Volume = {40},
	Year = {2012}}

@article{mckeague,
	Abstract = {{Summary: This paper develops a point impact linear regression model
    in which the trajectory of a continuous stochastic process, when evaluated
    at a sensitive time point, is associated with a scalar response. The
    proposed model complements and is more interpretable than the functional
    linear regression approach that has become popular in recent years. The
    trajectories are assumed to have fractal (self-similar) properties in common
    with a fractional Brownian motion with an unknown Hurst exponent. Bootstrap
    confidence intervals based on the least-squares estimator of the sensitive
    time point are developed. Misspecification of the point impact model by a
    functional linear model is also investigated. Non-Gaussian limit
    distributions and rates of convergence determined by the Hurst exponent play
    an important role.}},
	Author = {McKeague, Ian W. and Sen, Bodhisattva},
	Classmath = {{*62M10 (Time series, etc. (statistics)) 62G08 (Nonparametric regression) 62M09 (Non-Markovian processes: estimation) 62E20 (Asymptotic distribution theory in statistics) 62J05 (Linear regression) 60J65 (Brownian motion) }},
	Doi = {10.1214/10-AOS791},
	Journal = {Ann. Stat.},
	Keywords = {{functional linear regression; fractional Brownian motion; M-estimation; misspecification; nonstandard asymptotics; empirical processes; bootstrap methods}},
	Language = {English},
	Number = {4},
	Pages = {2559-2586},
	Title = {{Fractals with point impact in functional linear regression.}},
	Volume = {38},
	Year = {2010},
	Bdsk-Url-1 = {http://dx.doi.org/10.1214/10-AOS791}}

@article{hall_horowitz_2007,
	Abstract = {Summary: In functional linear regression, the slope ``parameter'' is a function. Therefore, in a nonparametric context, it is determined by an infinite number of unknowns. Its estimation involves solving an ill-posed problem and has points of contact with a range of methodologies, including statistical smoothing and deconvolution. The standard approach to estimating the slope function is based explicitly on functional principal components analysis and, consequently, on spectral decomposition in terms of eigenvalues and eigenfunctions. We discuss this approach in detail and show that in certain circumstances, optimal convergence rates are achieved by the PCA technique. An alternative approach based on quadratic regularisation is suggested and shown to have advantages from some points of view.},
	Author = {Hall, Peter and Horowitz, Joel L.},
	Doi = {10.1214/009053606000000957},
	Identifier = {1114.62048},
	Issn = {0090-5364},
	Journal = {The Annals of Statistics},
	Msc2010 = {62G08 (62H25 62G20 62J05)},
	Number = {1},
	Pages = {70-91},
	Publisher = {Institute of Mathematical Statistics, Beachwood, OH},
	Title = {Methodology and convergence rates for functional linear regression.},
	Volume = {35},
	Year = {2007},
	Bdsk-Url-1 = {http://dx.doi.org/10.1214/009053606000000957}}

@article{candes2011,
	Acmid = {1970395},
	Address = {New York, NY, USA},
	Articleno = {11},
	Author = {Cand\`{e}s, Emmanuel J. and Li, Xiaodong and Ma, Yi and Wright, John},
	Doi = {10.1145/1970392.1970395},
	Issn = {0004-5411},
	Issue_Date = {May 2011},
	Journal = {J. ACM},
	Keywords = {\?1-norm minimization, Principal components, duality, low-rank matrices, nuclear-norm minimization, robustness vis-a-vis outliers, sparsity, video surveillance},
	Month = jun,
	Number = {3},
	Numpages = {37},
	Pages = {11:1--11:37},
	Publisher = {ACM},
	Title = {Robust principal component analysis?},
	Url = {http://doi.acm.org/10.1145/1970392.1970395},
	Volume = {58},
	Year = {2011},
	Bdsk-Url-1 = {http://doi.acm.org/10.1145/1970392.1970395},
	Bdsk-Url-2 = {http://dx.doi.org/10.1145/1970392.1970395}}

@article{RPCA,
	Author = {E.J. Cand\`es and X. Li and Y. Ma and J. Wright},
	Journal = {Journal of the ACM},
	Number = {3},
	Title = {Robust principal component analysis?},
	Volume = {58},
	Year = {2011}}

@article{anto1,
	Author = {A. Antoniadis},
	Journal = {Statistics Surveys},
	Title = {Wavelet methods in statistics: Some recent developments and their applications},
	Volume = {1},
	Year = {2007}}

@article{morris1,
	Author = {J.S. Morris},
	Journal = {Journal of the Royal Statistical Society: Series B},
	Title = {Wavelet-based functional mixed models},
	Volume = {68},
	Year = {2006}}

@article{morris2,
	Author = {J.S. Morris and M. Vannucci and P.J. Brown and R.J. Caroll},
	Journal = {Journal of the American Statistical Association},
	Title = {Wavelet-based nonparametric modelling of hierarchical functions in colon carcinogenesis},
	Volume = {98},
	Year = {2003a}}

@article{morris3,
	Author = {J.S. Morris and M. Vannucci and P.J. Brown and R.J. Caroll},
	Journal = {Journal of the American Statistical Association},
	Title = {Discussion on ``Wavelet-based nonparametric modelling of hierarchical functions in colon carcinogenesis"},
	Volume = {98},
	Year = {2003b}}

@article{luo,
	Author = {X. Luo},
	Journal = {JRSSB, under review},
	Title = {High dimensional covariance matrix estimation via convex minimization},
	Year = {2011}}

@book{RamSIl,
	Author = {J.O. Ramsay and B.W. Silverman},
	Publisher = {Springer, New-York},
	Title = {Functional Data Analysis},
	Year = {2005}}

@book{RamSIl2,
	Author = {J.O. Ramsay and B.W. Silverman},
	Publisher = {Springer, New-York},
	Title = {Applied Functional Data Analysis: Methods and Case Studies},
	Year = {2002}}

@book{HorKok,
	Author = {L. Horvath and P. Kokoszka},
	Publisher = {Springer Series in Statistics},
	Title = {Inference for Functional Data with Applications},
	Year = {2012}}

@book{bosq,
	Author = {D. Bosq},
	Publisher = {Springer-Verlag New-York},
	Title = {Linear Processes in Function Spaces},
	Year = {2000}}

@book{Mallat,
	Author = {S. Mallat},
	Publisher = {Academic Press},
	Title = {A Wavelet Tour of Signal Processing},
	Year = {2008}}

@article{caiYuan1,
	Author = {T.T. Cai and M. Yuan},
	Journal = {The Annals of Statistics},
	Number = {4},
	Title = {Adaptative covariance matrix estimation through block thresholding},
	Volume = {40},
	Year = {2012}}

@article{Bickel,
	Author = {P.J. Bickel and E. Levina},
	Journal = {The Annals of Statistics},
	Number = {1},
	Title = {Regularized estimation of large covariance matrices},
	Volume = {36},
	Year = {2008}}

@article{silver1,
	Author = {B.W. Silverman},
	Journal = {The Annals of Statistics},
	Number = {1},
	Title = {Smoothed functional principal components analysis by choice of norm},
	Volume = {24},
	Year = {1996}}

@article{caiYuan2,
	Author = {T.T. Cai and M. Yuan},
	Journal = {Technical report},
	Title = {Nonparametric covariance function estimation for functional and longitudinal data},
	Year = {2010}}

@article{amini,
	Author = {A.A. Amini and M.J. Wainwright},
	Journal = {The Annals of Statistics},
	Number = {5},
	Title = {Sampled forms of functional PCA in reproducing kernel Hibert spaces},
	Volume = {40},
	Year = {2012}}

@article{LiuVanden,
	Author = {Z. Liu and L. Vandenberghe},
	Journal = {Journal on Matrix Analysis and Applications},
	Number = {3},
	Title = {Interior-point method for nuclear norm approximation with application to system identification},
	Volume = {31},
	Year = {2009}}

@phdthesis{Fazel,
	Author = {M. fazel},
	School = {Stanford University},
	Title = {Matrix rank minimization with applications},
	Year = {2002}}

@incollection{mas-menneteau:2003,
	Author = {Mas, A. and Menneteau, L.},
	Booktitle = {High Dimensional Probability III},
	Date-Added = {2012-11-16 13:59:32 +0000},
	Date-Modified = {2012-11-16 14:00:47 +0000},
	Journal = {Progress in Probability},
	Number = {1},
	Pages = {127--133},
	Publisher = {Birkh{\"a}user},
	Title = {Perturbation approach applied to the asymptotic study of random operators},
	Volume = {55},
	Year = {2003}}

@article{cramer:1942,
	Author = {Cram\'er, Harald},
	Date-Added = {2012-11-26 15:35:38 +0100},
	Date-Modified = {2012-11-26 15:36:13 +0100},
	Journal = {Ark. Mat. Astron. Fys.},
	Pages = {1-7},
	Title = {On harmonic analysis in certain functional spaces},
	Volume = {28B},
	Year = {1942}}

@book{Steele:2003,
	Address = {New York},
	Author = {Steele, J. Michael},
	Date-Added = {2012-11-16 15:18:33 +0000},
	Date-Modified = {2012-11-16 15:18:40 +0000},
	Edition = {Corr. 3rd printing},
	Isbn = {0-387-95016-8},
	Publisher = {Springer},
	Series = {Stochastic modelling and applied probability},
	Title = {Stochastic calculus and financial applications},
	Volume = {45, 3rd corr. pr},
	Year = {2003}}

@book{Dinculeanu:2000,
	Address = {New York},
	Author = {Dinculeanu, Nicolae},
	Date-Added = {2012-11-16 15:01:02 +0000},
	Date-Modified = {2012-11-16 15:01:10 +0000},
	Isbn = {0-471-37738-4},
	Publisher = {Wiley},
	Series = {Pure and applied mathematics},
	Title = {Vector integration and stochastic integration in Banach spaces},
	Year = {2000}}

@inproceedings{brislawn:1988,
	Author = {Brislawn, C.},
	Booktitle = {Proc. Am. Math. Soc},
	Date-Added = {2012-11-16 14:01:11 +0000},
	Date-Modified = {2012-11-16 14:01:25 +0000},
	Pages = {1181--1190},
	Title = {Kernels of trace class operators},
	Volume = {104},
	Year = {1988}}

@article{mas:2009,
	Author = {Mas, Andr\'e and Pumo, Besnik},
	Date-Added = {2012-11-25 15:10:37 +0100},
	Date-Modified = {2012-11-25 15:11:20 +0100},
	Journal = {Arxiv preprint arXiv:0901.2503},
	Title = {Linear Processes for Functional Data},
	Year = {2009}}

@article{kokoszka:2012,
	Author = {Kokoszka, Piotr},
	Date-Added = {2012-11-25 15:07:23 +0100},
	Date-Modified = {2012-11-25 15:09:29 +0100},
	Journal = {ISRN Probability and Statistics},
	Title = {Dependent Functional Data},
	Volume = {2012},
	Year = {2012}}

@book{ferraty:2011,
	Author = {Ferraty, F. and Romain, Y.},
	Date-Added = {2012-11-25 15:03:02 +0100},
	Date-Modified = {2012-11-25 15:05:49 +0100},
	Publisher = {Oxford University Press},
	Title = {The Oxford Handbook of Functional Data Analysis},
	Year = {2011}}

@article{wainwright:2011,
	Author = {Amini, Arash. A. and Wainwright, Martin J.},
	Journal = {Annals of Statistics},
	Number = {5},
	Pages = {2452-2482},
	Title = {Sampled forms of functional PCA in reproducing kernel Hilbert spaces},
	Volume = {40},
	Year = {2012}}

@article{yao:2005b,
	Author = {Yao, F. and M{{\"u}}ller, H. G. and Wang, J. L.},
	Date-Added = {2012-11-25 14:55:50 +0100},
	Date-Modified = {2012-11-25 14:57:01 +0100},
	Journal = {Journal of the American Statistical Association},
	Pages = {577-590},
	Title = {Functional Data Analysis of Sparse Longitudinal Data},
	Volume = {100},
	Year = {2005}}

@article{hall_etal:2006,
	Author = {Hall, Peter and M{{\"u}}ller, H. G. and Wang, J. L.},
	Date-Added = {2012-11-25 14:48:38 +0100},
	Date-Modified = {2012-11-25 14:49:43 +0100},
	Journal = {Annals of Statistics},
	Number = {3},
	Pages = {1493-1517},
	Title = {Properties of principal component methods for functional and longitudinal data analysis},
	Volume = {34},
	Year = {2006}}

@article{silverman:1996,
	Author = {Silverman, B. W},
	Date-Added = {2012-11-25 14:47:02 +0100},
	Date-Modified = {2012-11-25 14:47:41 +0100},
	Journal = {Annals of Statistics},
	Number = {1},
	Pages = {1-24},
	Title = {Smoothed functional principal components analysis by choice of norm},
	Volume = {24},
	Year = {1996}}

@article{cardot:2000,
	Author = {Cardot, Herv{\'e}},
	Date-Added = {2012-11-25 14:45:45 +0100},
	Date-Modified = {2012-11-25 14:46:15 +0100},
	Journal = {Journal of Nonparametric Statistics},
	Pages = {503-538},
	Title = {Nonparametric Estimation of Smoothed Principal Components Analysis of Sampled Noisy Functions},
	Volume = {12},
	Year = {2000}}

@article{cardot:2007,
	Author = {Cardot, Herv{\'e}},
	Date-Added = {2012-11-25 14:43:47 +0100},
	Date-Modified = {2012-11-25 14:44:22 +0100},
	Journal = {Scandinavian Journal of Statistics},
	Number = {2},
	Pages = {317-335},
	Title = {Conditional Functional Principal Components Analysis},
	Volume = {34},
	Year = {2007}}

@article{hall:2009,
	Author = {Hall, Peter and Hosseini-Nasab, Mohammad},
	Date-Added = {2012-11-25 14:41:52 +0100},
	Date-Modified = {2012-11-25 14:42:43 +0100},
	Journal = {Mathematical Proceedings of the Cambridge Philosophical Society},
	Number = {1},
	Pages = {225-256},
	Title = {Theory for high-order bounds in functional principal components analysis},
	Volume = {146},
	Year = {2009}}

@article{mas:2002,
	Author = {Mas, Andr\'e},
	Date-Added = {2012-11-25 14:01:12 +0100},
	Date-Modified = {2012-11-25 14:01:48 +0100},
	Journal = {Stochastic Processes and their Applications},
	Pages = {117-135},
	Title = {Weak convergence for the covariance operators of a Hilbertian linear process},
	Volume = {99},
	Year = {2002}}

@article{bosq:1990,
	Author = {Bosq, Denis},
	Date-Added = {2012-11-25 13:54:50 +0100},
	Date-Modified = {2012-11-25 13:55:57 +0100},
	Journal = {Comptes Rendus de l'Acad\'emie des Sciences. S\'erie I},
	Number = {11},
	Pages = {787-790},
	Title = {Mod\`ele autor\'egressif hilbertien. Application \`a la pr\'evision du comportement d'un processus \'a temps continu sur un intervalle de temps donn\'e.},
	Volume = {310},
	Year = {1990}}

@article{bosq:1989,
	Abstract = {Summary: We study the empirical covariance operator and the empirical crossed covariance operator associated with a Hilbertian strong mixing stationary process. Interpreting these operators as random variables in the Hilbert- Schmidt operators space we obtain several results: optimality, almost sure convergence, limit laws, estimation of theoretical eigenvalues and eigenvectors, rates of convergence.},
	Author = {Bosq, Denis},
	Date-Modified = {2012-11-25 13:52:36 +0100},
	Identifier = {0683.62055},
	Issn = {0764-4442},
	Journal = {Comptes Rendus de l'Acad\'emie des Sciences. S\'erie I},
	Msc2010 = {62M99 (60B11 60B12)},
	Number = {14},
	Pages = {873-875},
	Publisher = {Elsevier, Paris},
	Title = {Propri\'et\'es des op\'erateurs de covariance empiriques d'un processus stationnaire hilbertien.},
	Volume = {309},
	Year = {1989}}

@article{besse:1986,
	Author = {Besse, P. and Ramsay, James O},
	Date-Added = {2012-11-15 20:12:15 +0000},
	Date-Modified = {2012-11-15 20:13:14 +0000},
	Journal = {Psychometrika},
	Pages = {285-311},
	Title = {Principal components-analysis of sampled functions.},
	Volume = {51},
	Year = {1986}}

@article{kleffe:1973,
	Author = {Kleffe, J{\"u}rgen},
	Date-Added = {2012-11-15 18:53:22 +0000},
	Date-Modified = {2012-11-15 18:53:40 +0000},
	Journal = {Mathematische Operationsforschung Statistik},
	Number = {5},
	Pages = {391-406},
	Title = {Principal components of random variables with values in a seperable hilbert space},
	Volume = {4},
	Year = {1973},
	Bdsk-Url-1 = {http://www.tandfonline.com/doi/abs/10.1080/02331887308801137},
	Bdsk-Url-2 = {http://dx.doi.org/10.1080/02331887308801137}}

@article{rao:1958,
	Author = {Rao, C. Radhakrishna},
	Copyright = {Copyright {\copyright} 1958 International Biometric Society},
	Date-Modified = {2012-11-14 21:16:17 +0000},
	Issn = {0006341X},
	Journal = {Biometrics},
	Jstor_Articletype = {research-article},
	Jstor_Formatteddate = {Mar., 1958},
	Language = {English},
	Number = {1},
	Pages = {pp. 1-17},
	Publisher = {International Biometric Society},
	Title = {Some Statistical Methods for Comparison of Growth Curves},
	Url = {http://www.jstor.org/stable/2527726},
	Volume = {14},
	Year = {1958},
	Bdsk-Url-1 = {http://www.jstor.org/stable/2527726}}

@article{grenander:1950,
	Author = {Grenander, Ulf},
	Date-Added = {2012-11-14 20:56:59 +0000},
	Date-Modified = {2012-11-14 20:58:06 +0000},
	Issn = {0004-2080},
	Issue = {3},
	Journal = {Arkiv f{\"o}r Matematik},
	Keyword = {Mathematics and Statistics},
	Pages = {195-277},
	Publisher = {Springer Netherlands},
	Title = {Stochastic processes and statistical inference},
	Url = {http://dx.doi.org/10.1007/BF02590638},
	Volume = {1},
	Year = {1950},
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/BF02590638}}

@article{Horvath:10a,
	Author = {Horv\'{a}th, L. and Hu\v{s}kov\'{a}, M. and Kokoszka, P.},
	Date-Added = {2012-09-28 10:06:06 +0200},
	Date-Modified = {2012-09-29 11:40:39 +0000},
	Journal = {Journal of Multivariate Analysis},
	Pages = {352--367},
	Title = {Testing the Stability of the Functional Autoregressive Process},
	Volume = {101},
	Year = {2010}}

@article{main-paper,
	Author = {Panaretos, V. M. and Tavakoli, S.},
	Date-Added = {2012-09-24 18:52:58 +0200},
	Date-Modified = {2012-09-24 18:54:16 +0200},
	Title = {{Fourier Analysis of Stationary Time Series in Function Space}},
	Year = {2012}}

@article{supplement,
	Author = {Panaretos, V. M. and Tavakoli, S.},
	Date-Added = {2012-09-24 18:27:13 +0200},
	Date-Modified = {2012-09-24 18:44:51 +0200},
	Title = {{Supplement to ``Fourier Analysis of Stationary Time Series in Function Space''}},
	Year = {2012}}

@book{kolmogorov:1978,
	Author = {Kolmogorov, A.N.},
	Date-Added = {2012-09-24 00:36:38 +0200},
	Date-Modified = {2012-09-24 00:36:48 +0200},
	Publisher = {John Crerar Library] National Translations Center},
	Title = {Stationary sequences in Hilbert space},
	Year = {1978}}

@article{louani:2010,
	Author = {Laib, N. and Louani, D.},
	Date-Added = {2012-09-07 13:21:54 +0000},
	Date-Modified = {2012-09-07 13:22:05 +0000},
	Journal = {Journal of Multivariate Analysis},
	Number = {10},
	Pages = {2266--2281},
	Publisher = {Elsevier},
	Title = {Nonparametric kernel regression estimation for functional stationary ergodic data: Asymptotic properties},
	Volume = {101},
	Year = {2010}}

@article{ferraty-tadj:2011,
	Author = {Ferraty, F. and Laksaci, A. and Tadj, A. and Vieu, P.},
	Date-Added = {2012-09-07 13:19:05 +0000},
	Date-Modified = {2012-09-07 13:19:16 +0000},
	Journal = {Electronic Journal of Statistics},
	Pages = {159--171},
	Publisher = {Institute of Mathematical Statistics},
	Title = {Kernel regression with functional response},
	Volume = {5},
	Year = {2011}}

@article{ferraty-goia:2011,
	Author = {Ferraty, F. and Goia, A. and Salinelli, E. and Vieu, P.},
	Date-Added = {2012-09-07 13:11:13 +0000},
	Date-Modified = {2012-09-07 13:11:43 +0000},
	Journal = {Recent Advances in Functional Data Analysis and Related Topics},
	Pages = {97--102},
	Publisher = {Springer},
	Title = {Recent Advances on Functional Additive Regression},
	Year = {2011}}

@book{Hunter:2005,
	Address = {Hackensack, N.J},
	Author = {Hunter, John K and Nachtergaele, Bruno},
	Call-Number = {QA300},
	Date-Added = {2012-09-06 16:28:45 +0000},
	Date-Modified = {2012-09-06 16:29:08 +0000},
	Dewey-Call-Number = {515},
	Edition = {Reprint},
	Publisher = {World Scientific},
	Title = {Applied analysis},
	Year = {2005}}

@article{Horvath:11,
	Author = {Horv\'{a}th, L. and Kokoszka, Piotr and Reeder, R.},
	Date-Added = {2012-09-06 15:54:29 +0000},
	Date-Modified = {2012-09-06 15:55:31 +0000},
	Doi = {10.1111/j.1467-9868.2012.01032.x},
	Issn = {1467-9868},
	Journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
	Keywords = {Eurodollar futures, Functional data analysis, Long-run variance, Time series, Two-sample problem},
	Pages = {no--no},
	Publisher = {Blackwell Publishing Ltd},
	Title = {Estimation of the mean of functional time series and a two-sample problem},
	Url = {http://dx.doi.org/10.1111/j.1467-9868.2012.01032.x},
	Year = {2012},
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1467-9868.2012.01032.x}}

@article{Hall:2007,
	Author = {Hall, P. and Van Keilegom, I.},
	Date-Added = {2012-09-06 15:50:57 +0000},
	Date-Modified = {2012-09-06 15:51:10 +0000},
	Journal = {Statistica Sinica},
	Number = {4},
	Pages = {1511},
	Title = {Two-sample tests in functional data analysis starting from discrete data},
	Volume = {17},
	Year = {2007}}

@article{Fremdt:2011,
	Author = {Fremdt, S. and Horv{\'a}th, L. and Kokoszka, P. and Steinebach, J.G.},
	Date-Added = {2012-09-06 15:50:10 +0000},
	Date-Modified = {2012-09-06 15:50:19 +0000},
	Journal = {Arxiv preprint arXiv:1104.4049},
	Title = {Testing the Equality of Covariance Operators in Functional Samples},
	Year = {2011}}

@article{Boente:2011,
	Author = {Boente, G. and Rodriguez, D. and Sued, M.},
	Date-Added = {2012-09-06 15:48:49 +0000},
	Date-Modified = {2012-09-06 15:49:01 +0000},
	Journal = {Recent Advances in Functional Data Analysis and Related Topics},
	Pages = {49--53},
	Publisher = {Springer},
	Title = {Testing the Equality of Covariance Operators},
	Year = {2011}}

@book{Horvath:2012,
	Address = {New York, NY},
	Author = {Horv{\'a}th, Lajos and Kokoszka, Piotr},
	Call-Number = {QA320},
	Date-Added = {2012-09-06 15:20:36 +0000},
	Date-Modified = {2012-09-06 15:21:08 +0000},
	Genre = {Functional analysis},
	Isbn = {978-1-4614-3654-6},
	Publisher = {Springer},
	Series = {Springer series in statistics},
	Title = {Inference for functional data with applications},
	Year = {2012},
	Bdsk-Url-1 = {http://sfx.ethz.ch/sfx_locater?sid=ALEPH:EBI01&genre=book&isbn=9781461436546}}

@book{Anderson:1994,
	Address = {New York},
	Author = {Anderson, T.W},
	Date-Added = {2012-08-24 13:12:18 +0000},
	Date-Modified = {2012-08-24 13:23:12 +0000},
	Isbn = {0-471-04745-7},
	Library-Id = {70-126222},
	Publisher = {Wiley},
	Series = {Wiley classics library},
	Title = {The statistical analysis of time series},
	Year = {1994},
	Bdsk-Url-1 = {http://sfx.ethz.ch/sfx_locater?sid=ALEPH:EBI01&genre=book&isbn=9781118186428}}

@book{Hannan:1970,
	Address = {New York (N.Y.)},
	Author = {Hannan, Edward James},
	Date-Added = {2012-08-24 13:10:44 +0000},
	Date-Modified = {2012-08-24 13:22:48 +0000},
	Isbn = {0-471-34805-8},
	Publisher = {Wiley},
	Series = {Wiley series in probability and mathematical statistics},
	Title = {Multiple time series},
	Year = {1970},
	Bdsk-Url-1 = {http://sfx.ethz.ch/sfx_locater?sid=ALEPH:EBI01&genre=book&isbn=9780471348054&id=doi:10.1002/9780470316429}}

@article{Rosenblatt:1984,
	Author = {Rosenblatt, M.},
	Date-Added = {2012-08-24 13:08:21 +0000},
	Date-Modified = {2012-08-24 13:08:33 +0000},
	Doi = {10.1214/aop/1176993146},
	Journal = {Ann. Probab.},
	Pages = {1167-1180},
	Title = {{Asymptotic normality, strong mixing and spectral density estimates.}},
	Volume = {12},
	Year = {1984},
	Bdsk-Url-1 = {http://www.zentralblatt-math.org/zmath/en/search/?format=complete&q=an:0545.62058},
	Bdsk-Url-2 = {http://dx.doi.org/10.1214/aop/1176993146}}

@article{peligrad-wu:2010,
	Author = {Peligrad, Magda and Wu, Wei Biao},
	Date-Added = {2012-08-24 13:05:26 +0000},
	Date-Modified = {2012-08-24 13:05:36 +0000},
	Doi = {10.1214/10-AOP530},
	Journal = {Ann. Probab.},
	Number = {5},
	Pages = {2009-2022},
	Title = {{Central limit theorem for Fourier transforms of stationary processes.}},
	Volume = {38},
	Year = {2010},
	Bdsk-Url-1 = {http://www.zentralblatt-math.org/zmath/en/search/?format=complete&q=an:1206.60026},
	Bdsk-Url-2 = {http://dx.doi.org/10.1214/10-AOP530}}

@article{liu-wu:2010,
	Author = {Liu, Weidong and Wu, Wei Biao},
	Date-Added = {2012-08-24 13:04:41 +0000},
	Date-Modified = {2012-08-24 13:05:01 +0000},
	Doi = {10.1017/S026646660999051X},
	Journal = {Econom. Theory},
	Number = {4},
	Pages = {1218-1245},
	Title = {{Asymptotics of spectral density estimates.}},
	Volume = {26},
	Year = {2010},
	Bdsk-Url-1 = {http://www.zentralblatt-math.org/zmath/en/search/?format=complete&q=an:pre05770037},
	Bdsk-Url-2 = {http://dx.doi.org/10.1017/S026646660999051X}}

@article{shao-wu:2007,
	Author = {Shao, Xiaofeng and Wu, Wei Biao},
	Date-Added = {2012-08-24 13:03:57 +0000},
	Date-Modified = {2012-08-24 13:04:07 +0000},
	Doi = {10.1214/009053606000001479},
	Journal = {Ann. Stat.},
	Number = {4},
	Pages = {1773-1801},
	Title = {{Asymptotic spectral theory for nonlinear time series.}},
	Volume = {35},
	Year = {2007},
	Bdsk-Url-1 = {http://www.zentralblatt-math.org/zmath/en/search/?format=complete&q=an:1147.62076},
	Bdsk-Url-2 = {http://dx.doi.org/10.1214/009053606000001479}}

@book{priestley:2001,
	Author = {Priestley, M. B.},
	Date-Added = {2012-04-06 15:20:25 +0000},
	Date-Modified = {2012-04-06 15:23:11 +0000},
	Publisher = {Academic Press},
	Title = {Spectral analysis and time series, Volumes I and II},
	Year = {2001}}

@book{bloomfield:2000,
	Author = {Bloomfield, P.},
	Date-Added = {2012-04-06 15:14:40 +0000},
	Date-Modified = {2012-04-06 15:42:49 +0000},
	Publisher = {John Wiley \& Sons},
	Series = {Wiley Series in Probability and Statistics},
	Title = {Fourier analysis of Time Series: An Introduction},
	Year = {2000}}

@article{Panaretos:2012,
	Author = {Panaretos, V. M. and Tavakoli, S.},
	Date-Added = {2012-04-05 15:25:37 +0000},
	Date-Modified = {2013-03-08 20:07:52 +0000},
	Journal = {Annals of Statistics},
	Number = {2},
	Pages = {568--603},
	Title = {Fourier Analysis of Stationary Processes in Function Space},
	Volume = {41},
	Year = {2013}}

@book{Wand:1995,
	Address = {London},
	Author = {Wand, Matt P and Jones, M. Chris},
	Date-Added = {2012-04-02 12:03:46 +0000},
	Date-Modified = {2012-04-02 12:06:08 +0000},
	Isbn = {0-412-55270-1},
	Publisher = {Chapman \& Hall},
	Series = {Monographs on statistics and applied probability},
	Title = {Kernel smoothing},
	Volume = {60},
	Year = {1995}}

@article{hall:2006b,
	Author = {Hall, Peter and Vial, C{\'e}line},
	Date-Added = {2012-03-30 15:36:47 +0200},
	Date-Modified = {2012-03-30 15:37:14 +0200},
	Doi = {10.1111/j.1467-9868.2006.00562.x},
	Issn = {1467-9868},
	Journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
	Keywords = {Bootstrap, Confidence interval, Confounding, Degrees of freedom, Eigenvalue, Eigenvector, Functional data analysis, Hypothesis test, Low noise, Noise variance, Null hypothesis},
	Number = {4},
	Pages = {689--705},
	Publisher = {Blackwell Publishing Ltd},
	Title = {Assessing the finite dimensionality of functional data},
	Volume = {68},
	Year = {2006},
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1467-9868.2006.00562.x}}

@book{ferraty:2006,
	Author = {Ferraty, F. and Vieu, P.},
	Date-Added = {2012-03-29 11:32:46 +0200},
	Date-Modified = {2012-03-29 11:33:48 +0200},
	Publisher = {Springer},
	Title = {Nonparametric Functional Data Analysis: Theory and Practice},
	Year = {2006}}

@phdthesis{mas:2000,
	Author = {Mas, Andr\'e},
	Date-Added = {2012-03-29 11:13:43 +0200},
	Date-Modified = {2012-03-29 11:16:47 +0200},
	School = {Universit\'e Paris VI},
	Title = {Estimation d'op\'erateurs de corr\'elation de processus lin\'eaires fonctionnels: lois limites, d\'eviations mod\'er\'ees},
	Year = {2000}}

@book{Ledo:91,
	Author = {Michel Ledoux and Michel Talagrand},
	Date-Added = {2012-03-28 15:11:02 +0000},
	Date-Modified = {2012-03-28 15:11:02 +0000},
	Language = {English},
	Publisher = {{Ergebnisse der Mathematik und ihrer Grenzgebiete. 3. Folge, 23. Berlin etc.: Springer-Verlag. xii, 480 p. }},
	Title = {{Probability in Banach spaces. Isoperimetry and processes.}},
	Year = {1991}}

@book{Grenander:1966,
	Address = {New York},
	Author = {Grenander, Ulf and Rosenblatt, Murray},
	Date-Added = {2012-03-28 11:08:47 +0000},
	Date-Modified = {2012-03-28 15:06:54 +0000},
	Publisher = {J. Wiley},
	Title = {Statistical analysis of stationary time series},
	Year = {1966}}

@unpublished{Sen:10,
	Author = {Sen, R. and Kl{{\"u}}ppelberg, C.},
	Date-Added = {2012-03-28 07:40:44 +0000},
	Date-Modified = {2012-03-28 07:45:16 +0000},
	Note = {Unpublished manuscript, available online at},
	Title = {Time Series of Functional Data},
	Url = {http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.185.2739\&rep=rep1\&type=pdf},
	Bdsk-Url-1 = {http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.185.2739%5C&rep=rep1%5C&type=pdf}}

@article{kraus:2012,
	Annote = {Submitted},
	Author = {Kraus, D. and Panaretos, V. M.},
	Date-Added = {2012-03-28 07:29:47 +0000},
	Date-Modified = {2012-09-29 11:36:09 +0000},
	Journal = {Biometrika},
	Read = {0},
	Title = {Disperson operators and resistant second-order functional data analysis},
	Volume = {To appear.},
	Year = {2012}}

@incollection{loeve:1948,
	Author = {L\'evy, Paul},
	Booktitle = {{Processus stochastiques et mouvement brownien. Suivi d'une note de M. Lo\`eve. Levy, P.}},
	Classmath = {{*60-02 (Research monographs (probability theory)) 60Gxx (Stochastic processes) 60J65 (Brownian motion) }},
	Date-Added = {2012-03-28 07:26:21 +0000},
	Date-Modified = {2012-03-28 07:29:35 +0000},
	Keywords = {{Probability theory}},
	Language = {French},
	Publisher = {{Paris: Gauthier-Villars, \'Editeur 365 p. }},
	Reviewer = {{Szentm\'artony (Budapest)}},
	Title = {Fonctions al\'{e}atoires du seconde ordre},
	Year = {1948}}

@article{yao:2005,
	Author = {Yao, F. and M{{\"u}}ller, H. G. and Wang, J. L.},
	Citeulike-Article-Id = {2766847},
	Date-Added = {2012-03-28 07:20:53 +0000},
	Date-Modified = {2012-04-03 13:46:40 +0000},
	Journal = {Annals of Statistics},
	Keywords = {brisa},
	Number = {6},
	Pages = {2873--2903},
	Posted-At = {2008-05-07 16:43:21},
	Priority = {2},
	Title = {{Functional linear regression analysis for longitudinal data}},
	Volume = {33},
	Year = {2005}}

@article{rice:1991,
	Author = {John A. Rice and B.W. Silverman},
	Date-Added = {2012-03-28 07:18:19 +0000},
	Date-Modified = {2012-03-28 07:18:26 +0000},
	Journal = {J. R. Stat. Soc., Ser. B},
	Language = {English},
	Number = {1},
	Pages = {233--243},
	Title = {{Estimating the mean and covariance structure nonparametrically when the data are curves.}},
	Volume = {53},
	Year = {1991}}

@book{ramsay:2005,
	Author = {J.O. Ramsay and B.W. Silverman},
	Date-Added = {2012-03-28 07:17:47 +0000},
	Date-Modified = {2012-03-28 07:18:02 +0000},
	Edition = {2},
	Publisher = {Springer},
	Title = {Functional Data Analysis},
	Year = {2005}}

@book{ramsay:2002,
	Address = {New York},
	Author = {Ramsay, James O and Silverman, B. W},
	Date-Added = {2012-03-28 07:17:19 +0000},
	Date-Modified = {2012-03-28 15:07:36 +0000},
	Isbn = {0-387-95414-7},
	Publisher = {Springer},
	Series = {Springer series in statistics},
	Title = {Applied functional data analysis: methods and case studies},
	Url = {http://sfx.ethz.ch/sfx_locater?sid=ALEPH:EBI01&genre=book&isbn=978-0-387-95414-1&id=doi:10.1007/b98886},
	Year = {2002},
	Bdsk-Url-1 = {http://sfx.ethz.ch/sfx_locater?sid=ALEPH:EBI01&genre=book&isbn=978-0-387-95414-1&id=doi:10.1007/b98886}}

@article{panaretos:2010,
	Author = {V. M. Panaretos and D. Kraus and J. H. Maddocks},
	Date-Added = {2012-03-28 07:16:21 +0000},
	Date-Modified = {2012-03-28 07:16:31 +0000},
	Journal = {JASA Theory \& Methods},
	Month = {June},
	Number = {490},
	Pages = {670--682},
	Title = {Second-Order Comparison of Gaussian Random Functions and the Geometry of DNA Minicircles},
	Volume = {105},
	Year = {2010}}

@article{locantore:1999,
	Author = {Locantore, N. and Marron, J.S. and Simpson, D.G. and Tripoli, N. and Zhang, J.T. and Cohen, K.L.},
	Date-Added = {2012-03-27 20:51:00 +0200},
	Date-Modified = {2012-03-27 20:51:12 +0200},
	Doi = {10.1007/BF02595862},
	Journal = {Test},
	Number = {1},
	Pages = {1-73},
	Title = {{Robust principal component analysis for functional data. (With comments).}},
	Volume = {8},
	Year = {1999},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RElpOUy5vYmplY3RzViRjbGFzc1dOUy5rZXlzog8QgASABoAHohMUgAKAA1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgMGRpXTlMuZGF0YU8RAXwAAAAAAXwAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMq4/xRIKwAAAAvjnAxjaXRhdGlvbi5iaWIAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAKiuRzMluhQAAAAAAAAAAAAUAAgAACSAAAAAAAAAAAAAAAAAAAAAJRG93bmxvYWRzAAAQAAgAAMq5N1QAAAARAAgAAMzJtNUAAAABAAwAC+OcAAvjTwAAwCMAAgA1TWFjaW50b3NoIEhEOlVzZXJzOgBwYW5hcmV0bzoARG93bmxvYWRzOgBjaXRhdGlvbi5iaWIAAA4AGgAMAGMAaQB0AGEAdABpAG8AbgAuAGIAaQBiAA8AGgAMAE0AYQBjAGkAbgB0AG8AcwBoACAASABEABIAJVVzZXJzL3BhbmFyZXRvL0Rvd25sb2Fkcy9jaXRhdGlvbi5iaWIAABMAAS8AABUAAgAP//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfECUuLi8uLi8uLi8uLi8uLi9Eb3dubG9hZHMvY2l0YXRpb24uYmli0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBkAGwAbwBxAHMAdQB4AHoAfACGAJMAmACgAiACIgInAjACOwI/Ak0CVAJdAoUCigKNApoCnwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKx},
	Bdsk-Url-1 = {http://www.zentralblatt-math.org/zmath/en/search/?format=complete&q=an:0980.62049},
	Bdsk-Url-2 = {http://dx.doi.org/10.1007/BF02595862}}

@article{karhunen:1947,
	Author = {Karhunen, Kari},
	Date-Added = {2012-03-27 20:50:03 +0200},
	Date-Modified = {2012-03-27 20:50:15 +0200},
	Journal = {Ann. Acad. Sci. Fenn., Ser. A I, No.},
	Pages = {79 p.},
	Title = {{{\"U}ber lineare Methoden in der Wahrscheinlichkeitsrechnung.}},
	Volume = {37},
	Year = {1947},
	Bdsk-Url-1 = {http://www.zentralblatt-math.org/zmath/en/search/?format=complete&q=an:0030.16502}}

@article{hall:2006,
	Author = {Hall, Peter and Hosseini-Nasab, Mohammad},
	Date-Added = {2012-03-27 20:49:26 +0200},
	Date-Modified = {2012-03-27 20:49:34 +0200},
	Doi = {10.1111/j.1467-9868.2005.00535.x},
	Journal = {J. R. Stat. Soc., Ser. B, Stat. Methodol.},
	Number = {1},
	Pages = {109-126},
	Title = {{On properties of functional principal components analysis.}},
	Volume = {68},
	Year = {2006},
	Bdsk-Url-1 = {http://www.zentralblatt-math.org/zmath/en/search/?format=complete&q=an:1141.62048},
	Bdsk-Url-2 = {http://dx.doi.org/10.1111/j.1467-9868.2005.00535.x}}

@book{grenander:1981,
	Author = {Grenander, Ulf},
	Date-Added = {2012-03-27 20:48:57 +0200},
	Date-Modified = {2012-03-27 20:49:08 +0200},
	Publisher = {{Wiley Series in Probability and Mathematical Statistics. New York etc.: John Wiley \&amp; Sons. IX, 526 p. \$ 35.00 }},
	Title = {{Abstract inference.}},
	Year = {1981},
	Bdsk-Url-1 = {http://www.zentralblatt-math.org/zmath/en/search/?format=complete&q=an:0505.62069}}

@article{dauxois:1982,
	Author = {Dauxois, J. and Pousse, A. and Romain, Y.},
	Date-Added = {2012-03-27 20:48:13 +0200},
	Date-Modified = {2012-03-27 20:48:23 +0200},
	Doi = {10.1016/0047-259X(82)90088-4},
	Journal = {J. Multivariate Anal.},
	Pages = {136-154},
	Title = {{Asymptotic theory for the principal component analysis of a vector random function: Some applications to statistical inference.}},
	Volume = {12},
	Year = {1982},
	Bdsk-Url-1 = {http://www.zentralblatt-math.org/zmath/en/search/?format=complete&q=an:0539.62064},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/0047-259X(82)90088-4}}

@article{cuevas:2002,
	Author = {Cuevas, Antonio and Febrero, Manuel and Fraiman, Ricardo},
	Date-Added = {2012-03-27 20:47:32 +0200},
	Date-Modified = {2012-03-27 20:47:42 +0200},
	Doi = {10.2307/3315952},
	Journal = {Can. J. Stat.},
	Number = {2},
	Pages = {285-300},
	Title = {{Linear functional regression: The case of fixed design and functional response.}},
	Volume = {30},
	Year = {2002},
	Bdsk-Url-1 = {http://www.zentralblatt-math.org/zmath/en/search/?format=complete&q=an:1012.62039},
	Bdsk-Url-2 = {http://dx.doi.org/10.2307/3315952}}

@misc{cardot:2003,
	Annote = {\href{www.quantlet.org/hizirjsp/sarda-cardot/sarda-cardot.pdf}},
	Author = {Cardot, Herv{\'e} and Sarda, Pascal},
	Date-Added = {2012-03-27 20:46:09 +0200},
	Date-Modified = {2012-03-27 20:46:58 +0200},
	Doi = {10.1007/3-7908-1701-5_4},
	Howpublished = {{Sperlich, Stephan (ed.) et al., The art of semiparametrics. Papers based on the presentation at the conference the art of semiparametrics, Berlin, Germany, October 18--23, 2006. Heidelberg: Physica-Verlag. Contributions to Statistics, 49-66 (2006).}},
	Title = {{Linear regression models for functional data.}},
	Year = {2006},
	Bdsk-Url-1 = {http://www.zentralblatt-math.org/zmath/en/search/?format=complete&q=an:pre05196624},
	Bdsk-Url-2 = {http://dx.doi.org/10.1007/3-7908-1701-5_4}}

@book{adler:1990,
	Author = {Adler, Robert J.},
	Date-Added = {2012-03-27 20:45:26 +0200},
	Date-Modified = {2012-03-27 20:45:38 +0200},
	Publisher = {{IMS Lecture Notes - Monograph Series. 12. Hayward, CA: Institute of Mathematical Statistics. vii, 160 p. }},
	Title = {{An introduction to continuity, extrema, and related topics for general Gaussian processes.}},
	Year = {1990},
	Bdsk-Url-1 = {http://www.zentralblatt-math.org/zmath/en/search/?format=complete&q=an:0747.60039}}




@article{benko:2009,
	Author = {Benko, Michal and H{\"a}rdle, Wolfgang and Kneip, Alois},
	Date-Added = {2012-03-27 20:44:37 +0200},
	Date-Modified = {2012-03-27 20:45:00 +0200},
	Doi = {10.1214/07-AOS516},
	Journal = {Ann. Stat.},
	Number = {1},
	Pages = {1-34},
	Title = {{Common functional principal components.}},
	Volume = {37},
	Year = {2009},
	Bdsk-Url-1 = {http://www.zentralblatt-math.org/zmath/en/search/?format=complete&q=an:1169.62057},
	Bdsk-Url-2 = {http://dx.doi.org/10.1214/07-AOS516}}

@article{bosq:2002,
	Affiliation = {Universit{\'e} Pierre et Marie Curie Paris France Paris France},
	Author = {Bosq, Denis},
	Date-Modified = {2012-04-03 13:47:32 +0000},
	Issn = {1387-0874},
	Issue = {3},
	Journal = {Statistical Inference for Stochastic Processes},
	Keyword = {Mathematics and Statistics},
	Note = {10.1023/A:1021279131053},
	Pages = {287-306},
	Publisher = {Springer Netherlands},
	Title = {Estimation of Mean and Covariance Operator of Autoregressive Processes in Banach Spaces},
	Volume = {5},
	Year = {2002},
	Bdsk-Url-1 = {http://dx.doi.org/10.1023/A:1021279131053}}

@article{cuevas:2004,
	Doi = {10.1016/j.csda.2003.10.021},
	Issn = {0167-9473},
	Journal = {Computational Statistics &amp; Data Analysis},
	Number = {1},
	Pages = {111 - 122},
	Title = {An anova test for functional data},
	Url = {http://www.sciencedirect.com/science/article/pii/S016794730300269X},
	Volume = {47},
	Year = {2004},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S016794730300269X},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.csda.2003.10.021}}

@article{dehling:2005,
	Author = {Dehling, Herold and Sharipov, Olimjon},
	Date-Modified = {2012-03-29 11:24:58 +0200},
	Journal = {Statistical Inference for Stochastic Processes},
	Number = {2},
	Pages = {137--149},
	Title = {Estimation of Mean and Covariance Operator for Banach Space Valued Autoregressive Processes with Dependent Innovations},
	Volume = {8},
	Year = {2005}}

@article{ferraty:2004,
	Author = {Ferraty, F. and Vieu, P.},
	Date-Modified = {2012-04-03 13:44:54 +0000},
	Doi = {10.1080/10485250310001622686},
	Journal = {Journal of Nonparametric Statistics},
	Number = {1-2},
	Pages = {111-125},
	Title = {Nonparametric models for functional data, with application in regression, time series prediction and curve discrimination},
	Volume = {16},
	Year = {2004},
	Bdsk-Url-1 = {http://www.tandfonline.com/doi/abs/10.1080/10485250310001622686},
	Bdsk-Url-2 = {http://dx.doi.org/10.1080/10485250310001622686}}

@article{kargin:2008,
	Author = {V. Kargin and A. Onatski},
	Doi = {10.1016/j.jmva.2008.03.001},
	Issn = {0047-259X},
	Journal = {Journal of Multivariate Analysis},
	Number = {10},
	Pages = {2508 - 2526},
	Title = {Curve forecasting by functional autoregression},
	Url = {http://www.sciencedirect.com/science/article/pii/S0047259X08000961},
	Volume = {99},
	Year = {2008},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0047259X08000961},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.jmva.2008.03.001}}

@article{mas:2007,
	Doi = {10.1016/j.jmva.2006.05.010},
	Issn = {0047-259X},
	Journal = {Journal of Multivariate Analysis},
	Number = {6},
	Pages = {1231 - 1261},
	Title = {Weak convergence in the functional autoregressive model},
	Url = {http://www.sciencedirect.com/science/article/pii/S0047259X0600090X},
	Volume = {98},
	Year = {2007},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0047259X0600090X},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.jmva.2006.05.010}}

@article{antoniadis:2009,
	Author = {Anestis Antoniadis and Efstathios Paparoditis and Theofanis Sapatinas},
	Date-Modified = {2012-04-03 13:47:33 +0000},
	Doi = {10.1016/j.spl.2008.10.028},
	Issn = {0167-7152},
	Journal = {Statistics &amp; Probability Letters},
	Number = {6},
	Pages = {733 - 740},
	Title = {Bandwidth selection for functional time series prediction},
	Volume = {79},
	Year = {2009},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0167715208005075},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.spl.2008.10.028}}

@article{antoniadis:2006,
	Author = {Antoniadis, Anestis and Paparoditis, Efstathios and Sapatinas, Theofanis},
	Date-Modified = {2012-04-03 13:47:33 +0000},
	Doi = {10.1111/j.1467-9868.2006.00569.x},
	Issn = {1467-9868},
	Journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
	Keywords = {alpha-mixing, Besov spaces, Exponential smoothing, Functional kernel regression, Pointwise prediction intervals, Resampling, Seasonal autoregressive integrated moving average models, Smoothing splines, Time series prediction, Wavelets},
	Number = {5},
	Pages = {837--857},
	Publisher = {Blackwell Publishing Ltd},
	Title = {A functional wavelet-kernel approach for time series prediction},
	Volume = {68},
	Year = {2006},
	Bdsk-Url-1 = {http://dx.doi.org/10.1111/j.1467-9868.2006.00569.x}}

@article{antoniadis:2003,
	Author = {Anestis Antoniadis and Theofanis Sapatinas},
	Date-Modified = {2012-04-03 13:47:33 +0000},
	Doi = {10.1016/S0047-259X(03)00028-9},
	Issn = {0047-259X},
	Journal = {Journal of Multivariate Analysis},
	Number = {1},
	Pages = {133 - 158},
	Title = {Wavelet methods for continuous-time prediction using Hilbert-valued autoregressive processes},
	Volume = {87},
	Year = {2003},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0047259X03000289},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/S0047-259X(03)00028-9}}

@unpublished{Horvath:11arxiv,
	Author = {Horv\'{a}th, L. and Kokoszka, Piotr and Reeder, R.},
	Date-Added = {2012-03-27 20:02:13 +0200},
	Date-Modified = {2012-09-06 15:55:31 +0000},
	Note = {arXiv:1105.0019v1 [math.ST]},
	Title = {Estimation of the mean of functional time series and a two sample problem},
	Url = {http://arxiv.org/abs/1105.0019v1},
	Year = {2011},
	Bdsk-Url-1 = {http://arxiv.org/abs/1105.0019v1}}

@article{Gabrys:2007,
	Author = {Gabrys, Robertas and Kokoszka, Piotr},
	Date-Added = {2012-03-27 19:59:47 +0200},
	Date-Modified = {2012-03-28 15:10:07 +0000},
	Journal = {Journal of the American Statistical Association},
	Pages = {1338-1348},
	Title = {Portmanteau Test of Independence for Functional Observations},
	Volume = {102},
	Year = {2007},
	Bdsk-Url-1 = {http://EconPapers.repec.org/RePEc:bes:jnlasa:v:102:y:2007:m:december:p:1338-1348},
	Bdsk-Url-2 = {http://econpapers.repec.org/article/besjnlasa/v_3a102_3ay_3a2007_3am_3adecember_3ap_3a1338-1348.htm}}

@book{Zhu:2007,
	Address = {Providence, RI},
	Annote = {talks about schatten classes
},
	Author = {Zhu, Kehe},
	Date-Added = {2012-03-23 17:36:41 +0000},
	Date-Modified = {2012-03-23 17:36:41 +0000},
	Edition = {2nd ed},
	Isbn = {978-0-8218-3965-2},
	Library-Id = {90-3738},
	Publisher = {American Mathematical Society},
	Series = {Mathematical surveys and monographs},
	Title = {Operator theory in function spaces},
	Volume = {vol. 138},
	Year = {2007}}

@book{Wheeden:1977,
	Address = {New York},
	Annote = {theory of function of bounded variation and riemann-stieltjes integrals},
	Author = {Wheeden, Richard L and Zygmund, Antoni Szczepan},
	Date-Added = {2012-03-23 17:36:33 +0000},
	Date-Modified = {2012-03-23 17:36:33 +0000},
	Isbn = {0-8247-6499-4},
	Publisher = {Dekker},
	Series = {Monographs and textbooks in pure and applied mathematics},
	Title = {Measure and integral: an introduction to real analysis},
	Volume = {vol. 43},
	Year = {1977}}

@book{Weid:80,
	Author = {Joachim Weidmann},
	Date-Added = {2012-03-23 17:36:28 +0000},
	Date-Modified = {2012-03-23 17:36:28 +0000},
	Language = {English},
	Publisher = {{Graduate Texts in Mathematics, Springer-Verlag}},
	Title = {{Linear operators in Hilbert spaces. Transl. by Joseph Sz{\"u}cs.}},
	Year = {1980}}

@book{Rudin:1976,
	Address = {New York},
	Author = {Rudin, Walter},
	Date-Added = {2012-03-23 17:36:12 +0000},
	Date-Modified = {2012-03-23 17:36:12 +0000},
	Edition = {3rd ed},
	Isbn = {0-07-054235-X},
	Publisher = {McGraw-Hill},
	Series = {International series in pure and applied mathematics},
	Title = {Principles of mathematical analysis},
	Year = {1976}}

@book{Rosenblatt:1985,
	Author = {Rosenblatt, Murray},
	Date-Added = {2012-03-23 17:35:55 +0000},
	Date-Modified = {2012-04-03 13:50:21 +0000},
	Isbn = {0-8176-3264-6},
	Publisher = {Birkh{\"a}user},
	Title = {Stationary sequences and random fields},
	Year = {1985}}

@book{Ringrose:1971,
	Address = {London},
	Annote = {talks about schatten classes},
	Author = {Ringrose, John R},
	Date-Added = {2012-03-23 17:35:50 +0000},
	Date-Modified = {2012-03-23 17:35:50 +0000},
	Isbn = {0-442-06956-1},
	Library-Id = {78-141984},
	Publisher = {van Nostrand Reinhold},
	Series = {van Nostrand Reinhold mathematical studies},
	Title = {Compact non-self-adjoint operators},
	Volume = {35},
	Year = {1971}}

@book{Polya:1972,
	Author = {G. P{{\'o}}lya and G. Szeg{{\"o}}},
	Date-Added = {2012-03-23 17:35:45 +0000},
	Date-Modified = {2012-03-23 17:35:45 +0000},
	Publisher = {{Springer-Verlag}},
	Title = {Problems and Theorems in Analysis},
	Volume = {1},
	Year = {1972}}

@book{Pollard:1984,
	Address = {New York},
	Author = {Pollard, D},
	Date-Added = {2012-03-23 17:35:38 +0000},
	Date-Modified = {2012-04-03 13:50:28 +0000},
	Isbn = {0387909907},
	Publisher = {Springer},
	Series = {Springer series in statistics},
	Title = {Convergence of stochastic processes},
	Year = {1984}}

@book{Munk:00,
	Author = {James R. Munkres},
	Date-Added = {2012-03-23 17:35:30 +0000},
	Date-Modified = {2012-03-23 17:35:30 +0000},
	Language = {English},
	Publisher = {{Prentice Hall}},
	Reviewer = {{Z.Karno (Bia{\l}ystok)}},
	Title = {{Topology. 2nd ed.}},
	Year = {2000}}

@book{Kadison:1997,
	Annote = {
},
	Author = {Kadison, Richard V and Ringrose, John R},
	Date-Added = {2012-03-23 17:35:22 +0000},
	Date-Modified = {2012-03-23 17:35:22 +0000},
	Library-Id = {97-20916},
	Publisher = {American Mathematical Society},
	Series = {Graduate studies in mathematics},
	Title = {Fundamentals of the theory of operator algebras},
	Year = {1997},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RElpOUy5vYmplY3RzViRjbGFzc1dOUy5rZXlzog8QgASABoAHohMUgAKAA1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgMGRpXTlMuZGF0YU8RAdwAAAAAAdwAAgAADE1hY2ludG9zaCBIRAAAAAAAAAAAAAAAAAAAAMgILv9IKwAAAA42VB8xMC4xMTExJTJGai4xNDY3LTk4NiMyNjZDRTcuYmliAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAJmzny5uDbQAAAAAAAAAAAAQAAgAACSAAAAAAAAAAAAAAAAAAAAAJRG93bmxvYWRzAAAQAAgAAMgIEt8AAAARAAgAAMubZ00AAAABAAwADjZUAA42RAAAk5YAAgBITWFjaW50b3NoIEhEOlVzZXJzOgBwYW5hcmV0bzoARG93bmxvYWRzOgAxMC4xMTExJTJGai4xNDY3LTk4NiMyNjZDRTcuYmliAA4ATgAmADEAMAAuADEAMQAxADEAJQAyAEYAagAuADEANAA2ADcALQA5ADgANgA4AC4AMgAwADAANgAuADAAMAA1ADYAMgAuAHgALgBiAGkAYgAPABoADABNAGEAYwBpAG4AdABvAHMAaAAgAEgARAASAD9Vc2Vycy9wYW5hcmV0by9Eb3dubG9hZHMvMTAuMTExMSUyRmouMTQ2Ny05ODY4LjIwMDYuMDA1NjIueC5iaWIAABMAAS8AABUAAgAP//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEDwuLi8uLi8uLi8uLi9Eb3dubG9hZHMvMTAuMTExMSUyRmouMTQ2Ny05ODY4LjIwMDYuMDA1NjIueC5iaWLSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGQAbABvAHEAcwB1AHgAegB8AIYAkwCYAKACgAKCAocCkAKbAp8CrQK0Ar0C/AMBAwQDEQMWAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAyg=}}

@article{Hormann:10,
	Author = {H{{\"o}}rmann, Siegfried and Kokoszka, Piotr},
	Coden = {ASTSC7},
	Date-Added = {2012-03-23 17:31:48 +0000},
	Date-Modified = {2012-04-03 13:45:39 +0000},
	Doi = {10.1214/09-AOS768},
	Fjournal = {The Annals of Statistics},
	Issn = {0090-5364},
	Journal = {Ann. Statist.},
	Mrclass = {62M10 (60G10 62G05)},
	Mrnumber = {2662361},
	Number = {3},
	Pages = {1845--1884},
	Title = {Weakly dependent functional data},
	Volume = {38},
	Year = {2010},
	Bdsk-Url-1 = {http://www.ams.org/mathscinet-getitem?mr=2662361},
	Bdsk-Url-2 = {http://dx.doi.org/10.1214/09-AOS768}}

@book{Hirsch:99,
	Address = {New York},
	Annote = {Really good!},
	Author = {Hirsch, Francis and Lacombe, Gilles},
	Date-Added = {2012-03-23 17:31:42 +0000},
	Date-Modified = {2012-03-23 17:31:42 +0000},
	Genre = {Funktionalanalysis},
	Isbn = {0387985247 Pp},
	Publisher = {Springer},
	Series = {Graduate texts in mathematics},
	Title = {Elements of functional analysis},
	Volume = {192},
	Year = {1999}}

@article{Gabrys:2010,
	Author = {Gabrys, Robertas and Lajos, Horv\'{a}th and Kokoszka, Piotr},
	Date-Added = {2012-03-23 17:31:23 +0000},
	Date-Modified = {2012-04-03 13:45:22 +0000},
	Journal = {Journal of the American Statistical Association},
	Number = {491},
	Pages = {1113-1125},
	Title = {Tests for Error Correlation in the Functional Linear Model},
	Volume = {105},
	Year = {2010},
	Bdsk-Url-1 = {http://EconPapers.repec.org/RePEc:bes:jnlasa:v:105:i:491:y:2010:p:1113-1125}}

@article{Ferreira:2009,
	Author = {Ferreira, Jos{\'e} C. and Menegatto, Valdir A. and Oliveira, Claudemir P.},
	Date-Added = {2012-03-23 17:28:02 +0000},
	Date-Modified = {2012-04-03 13:45:11 +0000},
	Doi = {10.1007/s11117-008-2240-9},
	Fjournal = {Positivity. An International Mathematics Journal Devoted to Theory and Applications of Positivity},
	Issn = {1385-1292},
	Journal = {Positivity},
	Mrclass = {47G10 (45H05 45P05 47B10)},
	Mrnumber = {2511239 (2010m:47061)},
	Mrreviewer = {Anton Schep},
	Number = {3},
	Pages = {519--541},
	Title = {On the nuclearity of integral operators},
	Volume = {13},
	Year = {2009},
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/s11117-008-2240-9}}

@book{Edwards:1967,
	Address = {New York},
	Author = {Edwards, R.E},
	Date-Added = {2012-03-23 17:27:52 +0000},
	Date-Modified = {2012-04-03 13:50:46 +0000},
	Publisher = {Holt, Rinehart \& Winston},
	Title = {Fourier series: a modern introduction},
	Year = {1967}}

@book{Blanke:2008,
	Author = {Bosq, D. and Blanke, D.},
	Date-Added = {2012-03-23 17:26:55 +0000},
	Date-Modified = {2012-09-06 15:17:50 +0000},
	Isbn = {9780470724026},
	Publisher = {John Wiley \& Sons},
	Read = {0},
	Series = {Wiley Series in Probability and Statistics},
	Title = {Inference and Prediction in Large Dimensions},
	Year = {2008},
	Bdsk-Url-1 = {http://books.google.com.pe/books?id=OMf9PcFR148C}}

@book{Bosq:00,
	Author = {D. Bosq},
	Date-Added = {2012-03-23 17:24:52 +0000},
	Date-Modified = {2012-03-23 17:24:52 +0000},
	Publisher = {Springer},
	Title = {Linear Processes in Function Spaces},
	Year = {2000}}

@book{hsing2015theoretical,
  title={Theoretical foundations of functional data analysis, with an introduction to linear operators},
  author={Hsing, Tailen and Eubank, Randall},
  year={2015},
  publisher={John Wiley \& Sons}
}

@misc{ramsay2005springer,
  title={Springer series in statistics},
  author={Ramsay, JO and Silverman, BW},
  journal={Functional data analysis},
  year={2005},
  publisher={Springer, c1997. New York}
}

@article{panaretos2013cramer,
  title={Cram{\'e}r--{K}arhunen--{L}o{\`e}ve representation and harmonic principal component analysis of functional time series},
  author={Panaretos, Victor M and Tavakoli, Shahin},
  journal={Stochastic Processes and their Applications},
  volume={123},
  number={7},
  pages={2779--2807},
  year={2013},
  publisher={Elsevier}
}

@article{descary2016functional,
  title={Functional Data Analysis by Matrix Completion},
  author={Descary, Marie-H{\'e}l{\`e}ne and Panaretos, Victor M},
  journal={arXiv preprint arXiv:1609.00834},
  year={2016}
}

@article{rippl2016limit,
  title={Limit laws of the empirical {W}asserstein distance: {G}aussian distributions},
  author={Rippl, Thomas and Munk, Axel and Sturm, Anja},
  journal={Journal of Multivariate Analysis},
  volume={151},
  pages={90--109},
  year={2016},
  publisher={Elsevier}
}

@article{yao2005functional2,
  title={Functional linear regression analysis for longitudinal data},
  author={Yao, Fang and M{\"u}ller, Hans-Georg and Wang, Jane-Ling and others},
  journal={The Annals of Statistics},
  volume={33},
  number={6},
  pages={2873--2903},
  year={2005},
  publisher={Institute of Mathematical Statistics}
}


@article{wang2016functional,
  title={Functional data analysis},
  author={Wang, Jane-Ling and Chiou, Jeng-Min and M{\"u}ller, Hans-Georg},
  journal={Annual Review of Statistics and Its Application},
  volume={3},
  pages={257--295},
  year={2016},
  publisher={Annual Reviews}
}

@article{alexander2005multiple,
  title={Multiple-fiber reconstruction algorithms for diffusion MRI},
  author={Alexander, Daniel C},
  journal={Annals of the New York Academy of Sciences},
  volume={1064},
  number={1},
  pages={113--133},
  year={2005},
  publisher={Wiley Online Library}
}

@article{von2009entropic,
  title={Entropic measure and {W}asserstein diffusion},
  author={von Renesse, Max-K and Sturm, Karl-Theodor},
  journal={The Annals of Probability},
  volume={37},
  number={3},
  pages={1114--1191},
  year={2009},
  publisher={Institute of Mathematical Statistics}
}


@article{schwartzman2008false,
  title={False discovery rate analysis of brain diffusion direction maps},
  author={Schwartzman, Armin and Dougherty, Robert F and Taylor, Jonathan E},
  journal={The Annals of Applied Statistics},
  pages={153--175},
  year={2008},
  publisher={JSTOR}
}

@article{karcher1977riemannian,
  title={Riemannian center of mass and mollifier smoothing},
  author={Karcher, Hermann},
  journal={Communications on pure and applied mathematics},
  volume={30},
  number={5},
  pages={509--541},
  year={1977},
  publisher={Wiley Online Library}
}



@article{panaretos2010second,
  title={Second-order comparison of Gaussian random functions and the geometry of DNA minicircles},
  author={Panaretos, Victor M and Kraus, David and Maddocks, John H},
  journal={Journal of the American Statistical Association},
  volume={105},
  number={490},
  pages={670--682},
  year={2010},
  publisher={Taylor \& Francis}
}



@article{kraus2012dispersion,
  title={Dispersion operators and resistant second-order functional data analysis},
  author={Kraus, David and Panaretos, Victor M},
  journal={Biometrika},
  volume={99},
  number={4},
  pages={813--832},
  year={2012},
  publisher={Oxford University Press}
}

@article{hastie1995penalized,
  title={Penalized discriminant analysis},
  author={Hastie, Trevor and Buja, Andreas and Tibshirani, Robert},
  journal={The Annals of Statistics},
  volume={23},
  number={1},
  pages={73--102},
  year={1995},
  publisher={Institute of Mathematical Statistics}
}

@article{cuesta2010simple,
  title={A simple multiway ANOVA for functional data},
  author={Cuesta-Albertos, JA and Febrero-Bande, M},
  journal={Test},
  volume={19},
  number={3},
  pages={537--557},
  year={2010},
  publisher={Springer}
}

@article{gorecki2015comparison,
  title={A comparison of tests for the one-way ANOVA problem for functional data},
  author={G{\'o}recki, Tomasz and Smaga, {\L}ukasz},
  journal={Computational Statistics},
  volume={30},
  number={4},
  pages={987--1010},
  year={2015},
  publisher={Springer}
}

@article{benko2009common,
  title={Common functional principal components},
  author={Benko, Michal and H{\"a}rdle, Wolfgang and Kneip, Alois},
  journal={The Annals of Statistics},
  volume={37},
  number={1},
  pages={1--34},
  year={2009},
  publisher={Institute of Mathematical Statistics}
}

@article{boente2018testing,
  title={Testing equality between several populations covariance operators},
  author={Boente, Graciela and Rodriguez, Daniela and Sued, Mariela},
  journal={Annals of the Institute of Statistical Mathematics},
  volume={70},
  number={4},
  pages={919--950},
  year={2018},
  publisher={Springer}
}

@article{pigoli2018statistical,
  title={The statistical analysis of acoustic phonetic data: exploring differences between spoken Romance languages},
  author={Pigoli, Davide and Hadjipantelis, Pantelis Z and Coleman, John S and Aston, John AD},
  journal={Journal of the Royal Statistical Society: Series C (Applied Statistics)},
  volume={67},
  number={5},
  pages={1103--1145},
  year={2018},
  publisher={Wiley Online Library}
}


@article{paparoditis2016bootstrap,
  title={Bootstrap-based testing of equality of mean functions or equality of covariance operators for functional data},
  author={Paparoditis, Efstathios and Sapatinas, Theofanis},
  journal={Biometrika},
  volume={103},
  number={3},
  pages={727--733},
  year={2016},
publisher={Oxford University Press}
}

@article{cabassi2017permutation,
  title={Permutation tests for the equality of covariance operators of functional data with applications to evolutionary biology},
  author={Cabassi, Alessandra and Pigoli, Davide and Secchi, Piercesare and Carter, Patrick A},
  journal={Electronic Journal of Statistics},
  volume={11},
  number={2},
  pages={3815--3840},
  year={2017},
  publisher={Institute of Mathematical Statistics and Bernoulli Society}
}


@article{cabassi2016fdcov,
  title={fdcov: Analysis of Covariance Operators},
  author={Cabassi, A and Kashlak, AB},
  journal={R package version},
  volume={1},
  number={0},
  year={2016}
}


@article{anderson2006distance,
  title={Distance-based tests for homogeneity of multivariate dispersions},
  author={Anderson, Marti J},
  journal={Biometrics},
  volume={62},
  number={1},
  pages={245--253},
  year={2006},
  publisher={Wiley Online Library}
}

@article{roy1953heuristic,
  title={On a heuristic method of test construction and its use in multivariate analysis},
  author={Roy, Samarendra Nath},
  journal={The Annals of Mathematical Statistics},
  pages={220--238},
  year={1953},
  publisher={JSTOR}
}


@article{fernique1970integrabilite,
  title={Int{\'e}grabilit{\'e} des vecteurs gaussiens},
  author={Fernique, Xavier},
  journal={CR Acad. Sci. Paris Serie A},
  volume={270},
  pages={1698--1699},
  year={1970}
}

@article{feldman1958equivalence,
  title={Equivalence and perpendicularity of Gaussian processes.},
  author={Feldman, Jacob},
  journal={Pacific Journal of Mathematics},
  volume={8},
  number={4},
  pages={699--708},
  year={1958},
  publisher={Pacific Journal of Mathematics, A Non-profit Corporation}
}

@article{hajek1958property,
  title={A property of $ J $-divergences of marginal probability distributions},
  author={H{\'a}jek, Jaroslav},
  journal={Czechoslovak Mathematical Journal},
  volume={8},
  number={3},
  pages={460--463},
  year={1958},
  publisher={Institute of Mathematics, Academy of Sciences of the Czech Republic}
}

@article{yao2005functional,
  title={Functional data analysis for sparse longitudinal data},
  author={Yao, Fang and M{\"u}ller, Hans-Georg and Wang, Jane-Ling},
  journal={Journal of the American statistical association},
  volume={100},
  number={470},
  pages={577--590},
  year={2005},
  publisher={Taylor \& Francis}
}

@article{pesarin2010permutation,
  title={The permutation testing approach: a review},
  author={Pesarin, Fortunato and Salmaso, Luigi},
  journal={Statistica},
  volume={70},
  number={4},
  pages={481--509},
  year={2010}
}

@book{Brill:01,
	Author = {D. R. Brillinger},
	Date-Added = {2012-03-23 17:24:48 +0000},
	Date-Modified = {2012-03-23 17:40:23 +0000},
	Edition = {(classics edition)},
	Publisher = {SIAM},
	Series = {Classics in Applied Mathematics},
	Title = {Time Series: Data Analysis and Theory},
	Year = {2001}}

@article{kashlak2019inference,
  title={Inference on covariance operators via concentration inequalities: k-sample tests, classification, and clustering via Rademacher complexities},
  author={Kashlak, Adam B and Aston, John AD and Nickl, Richard},
  journal={Sankhya A},
  volume={81},
  number={1},
  pages={214--243},
  year={2019},
  publisher={Springer}
}

@article{pillai1955some,
  title={Some new test criteria in multivariate analysis},
  author={Pillai, KC Sreedharan},
  journal={The Annals of Mathematical Statistics},
  pages={117--121},
  year={1955},
  publisher={JSTOR}
}

@article{kiefer1965admissible,
  title={Admissible Bayes character of T2-, R2-, and other fully invariant tests for classical multivariate normal problems},
  author={Kiefer, J and Schwartz, R},
  journal={The Annals of Mathematical Statistics},
  pages={747--770},
  year={1965},
  publisher={JSTOR}
}

@article{giri1968tests,
  title={On tests of the equality of two covariance matrices},
  author={Giri, N},
  journal={The Annals of Mathematical Statistics},
  volume={39},
  number={1},
  pages={275--277},
  year={1968},
  publisher={JSTOR}
}

@article{rao1963discrimination,
  title={Discrimination of Gaussian processes},
  author={Rao, C Radhakrishna and Varadarajan, VS},
  journal={Sankhy{\=a}: The Indian Journal of Statistics, Series A},
  pages={303--330},
  year={1963},
  publisher={JSTOR}
}

@misc{ramsay2021package,
  title={Package ‘fda’},
  author={Ramsay, JO and Wickham, Hadley and Ramsay, Maintainer JO and deSolve, Suggests},
  year={2021},
  publisher={Citeseer}
}

@article{ramsay2014description,
  title={Description and processing of functional data arising from juggling trajectories},
  author={Ramsay, James O and Gribble, Paul and Kurtek, Sebastian},
  journal={Electronic Journal of Statistics},
  volume={8},
  number={2},
  pages={1811--1816},
  year={2014},
  publisher={Institute of Mathematical Statistics and Bernoulli Society}
}

@article{hlavka2022functional,
  title={Functional ANOVA based on empirical characteristic functionals},
  author={Hl{\'a}vka, Zden{\v{e}}k and Hlubinka, Daniel and Ko{\v{n}}asov{\'a}, Kate{\v{r}}ina},
  journal={Journal of Multivariate Analysis},
  volume={189},
  pages={104878},
  year={2022},
  publisher={Elsevier}
}

@article{koshy2022exploring,
  title={Exploring British accents: Modelling the trap--bath split with functional data analysis},
  author={Koshy, Aranya and Tavakoli, Shahin},
  journal={Journal of the Royal Statistical Society Series C: Applied Statistics},
  volume={71},
  number={4},
  pages={773--805},
  year={2022},
  publisher={Oxford University Press}
}

@article{panaretos2018discussion,
  title={Discussion of The statistical analysis of acoustic phonetic data: exploring differences between spoken Romance languages},
  author={Panaretos, Victor M},
  year={2018}
}

@comment{BibDesk Smart Groups{
<?xml version="1.0" encoding="UTF-8"?>
<!DOCTYPE plist PUBLIC "-//Apple//DTD PLIST 1.0//EN" "http://www.apple.com/DTDs/PropertyList-1.0.dtd">
<plist version="1.0">
<array>
	<dict>
		<key>conditions</key>
		<array>
			<dict>
				<key>comparison</key>
				<integer>0</integer>
				<key>key</key>
				<string>Date-Added</string>
				<key>value</key>
				<string></string>
				<key>version</key>
				<string>1</string>
			</dict>
		</array>
		<key>conjunction</key>
		<integer>0</integer>
		<key>group name</key>
		<string>latest added</string>
	</dict>
</array>
</plist>
}}

